Mechanised Hypersafety Proofs about Structured Data: Extended Version

Arrays are a fundamental abstraction to represent collections of data. It is often possible to exploit structural properties of the data stored in an array (e.g., repetition or sparsity) to develop a specialised representation optimised for space efficiency. Formally reasoning about correctness of manipulations with such structured data is challenging, as they are often composed of multiple loops with non-trivial invariants. In this work, we observe that specifications for structured data manipulations can be phrased as hypersafety properties, i.e., predicates that relate traces of $k$ programs. To turn this observation into an effective verification methodology, we developed the Logic for Graceful Tensor Manipulation (LGTM), a new Hoare-style relational separation logic for specifying and verifying computations over structured data. The key enabling idea of LGTM is that of parametrised hypersafety specifications that allow the number $k$ of the program components to depend on the program variables. We implemented LGTM as a foundational embedding into Coq, mechanising its rules, meta-theory, and the proof of soundness. Furthermore, we developed a library of domain-specific tactics that automate computer-aided hypersafety reasoning, resulting in pleasantly short proof scripts that enjoy a high degree of reuse. We argue for the effectiveness of relational reasoning about structured data in LGTM by specifying and mechanically proving correctness of 13 case studies including computations on compressed arrays and efficient operations over multiple kinds of sparse tensors.

==> Makefile <==
all: Makefile *.tex *.bib
	rm -f *.pyg
	pdflatex -shell-escape --jobname=paper paper
	bibtex paper -min-crossrefs=5
	pdflatex -shell-escape --jobname=paper paper
	pdflatex -shell-escape --jobname=paper paper

#	pdflatex -shell-escape --jobname=paper "\def\extflag{}\input{paper}"

cover: Makefile *.tex *.bib
	pdflatex cover-letter
	pdflatex cover-letter

quick: Makefile *.tex *.bib
	rm -f *.pyg
	pdflatex -shell-escape --jobname=paper paper

appendix: Makefile *.tex
	pdflatex -shell-escape --jobname=appendix appendix
#	bibtex paper-extended -min-crossrefs=5 
#	pdflatex -shell-escape --jobname=appendix appendix
	pdflatex -shell-escape --jobname=appendix appendix


clean:
	rm -rf *.pyg *.aux *.bbl *.blg *.log *.out *.rel _minted-paper paper.pdf paper.zip	paper.fdb_latexmk paper.fls appendix.pdf

.PHONY: all clean

zip:
	zip paper.zip Makefile *.tex *.png _minted-paper/* *.bbl *.sty *.cls references.bib frameit.sty llncs.cls figures/*.tex figures/*.pdf tables/*


==> case-full.tex <==
\section{Case Study: Sparse Tensor Multiplication (Full Proof)}
\label{sec:case-study-full}


\paragraph{Specifying sparse matrix/vector multiplication}
%
To specify the result of \code{spmspv} compactly, let us introduce
some convenient notation.
%
First, we will use $\Zero$ to denote a 0-filled vector of a suitable
size evident from the context.
%
Second, we will abbreviate the joint assertion about all required
arrays across multiple components, which are not being modified,
simply as $\arrs$:
%
\begin{equation*}
{\small{
\arrs \eqdef \arr{\tinds{m}(\cdot)}{\inds{m}} \str
\arr{\tvals{m}(\cdot)}{\vals{m}} \str \arr{\tinds{x}(\cdot)}{\inds{x}}
\str \arr{\tvals{x}(\cdot)}{\vals{x}}
}}  
\end{equation*}
%
The desired specification is encoded by the following hypersafety triple:
%
\begin{equation}
\label{eq:csr1}
{\small{
\hspec{\!\!\!
\begin{array}{c}
  \arr{ans(1)}{\Zero} 
  \\[2pt]
  \str~\arrs  
\end{array}
\!\!\!}    
\hmid{\!\!\!
  \begin{array}{c@{\ }c@{\ }l}
  1 : \mathtt{spmspv(m_{ind}, m_{val}, x_{ind}, x_{val}, ans)} 
  \\ [2pt]
  \angled{2, i, j}_{\!\!\!\!\tiny
    \begin{array}{l} i \in [0, M) \\ j \in [0,N) \end{array}} :  \mathtt{csrij(m_{ind}, m_{val},} i, j)
  \\ [2pt]
  \angled{3, j}_{j \in [0, N)} : \mathtt{svi(x_{ind}, x_{val},} i)
  \end{array}
\!}
\hspec{\!\!\!
\left.
\begin{array}{r}
- \\[2pt] \many{m} \\[2pt] \many{x}
\end{array}
\right|
\begin{array}{l}
\exists a, \arr{ans(1)}{a} \str
\\[2pt]
\pure{\forall i, a[i] = \sum_j \many{m}(i,j)\many{x}(j)} 
\\[2pt]
\str \arrs \str \top  
\end{array}
\!\!\!}
}}
\end{equation}
%
The first line of the post-condition states that the result of the
computation stored in the array \code{ans} of the first component is a
dense vector~$a$ of the size $M$, while the second line asserts, in
the common mathematical notation, that $a$ is a result of multiplying
the dense representation of the matrix $\many{m}$ by the corresponding
dense vector~$\many{x}$.
%
We slightly abuse the hyper-value notation by referring to elements of
$\many{m}$ in the post-condition as $\many{m}(i, j)$, assuming that the
natural lexicographic order on the elements of the corresponding index
set $\set{\angled{2, i, j}~|~ i \in [0, M), j \in [0,N)}$.

The proof is best explained in two steps, each
focusing on one of its loops.

\paragraph{Step 1: Top-level \code{for}-loop decomposition}

The body of \code{spmspv} is represented by a loop that iterates
through all rows of the matrix~$m$ via the variable~\code{i}:
%
\begin{equation}
\label{eq:csr2}
{\small{
\hspec{\!\!\!
\begin{array}{c}
  \arr{ans(1)}{\Zero} 
  \\[2pt]
  \str~\arrs  
\end{array}
\!\!\!}    
\hmid{\!\!\!
  \begin{array}{c@{\ }c@{\ }l}
  1 : \forl{i}{0}{|\inds{m}|}{p(i)}
  \\ [2pt]
  \angled{2, i, j}_{\!\!\!\!\tiny
    \begin{array}{l} i \in [0, M) \\ j \in [0,N) \end{array}} :  \mathtt{csrij(m_{ind}, m_{val},} i, j)
  \\ [2pt]
  \angled{3, j}_{j \in [0, N)} : \mathtt{svi(x_{ind}, x_{val},} j) 
  \end{array}
\!}
\hspec{\!\!\!
\left.
\begin{array}{r}
- \\[2pt] \many{m} \\[2pt] \many{x}
\end{array}
\right|
\begin{array}{l}
\exists a, \arr{ans(1)}{a} \str
\\[2pt]
\pure{\forall i, a[i] = \sum_j \many{m}(i,j)\many{x}(j)} 
\\[2pt]
\str \arrs \str \top  
\end{array}
\!\!\!}
}}
\end{equation}
%
Each iteration of the \code{for}-loop handles exactly one row of $m$,
computing the value of multiplying it by all values of~$x$, encoded
via \code{x_ind} and \code{x_val}.
%
To proceed with our proof, we employ the general form of the
\rulename{For} rule.
%
$\Ifor(i, \many{m}\many{x})$ for the \code{for}-loop as follows:
%
\begin{equation*}
{\small{
  \Ifor(i, \many{m}\many{x}) \eqdef  
  \bigstr_{k = 0}^{i - 1} \Ans(1) + k \mapsto \sum_j\many{m}(i,
  j)\many{x}(j) \str
  \bigstr_{k = i}^{M - 1} \Ans(1) + k \mapsto 0
}}
\end{equation*}
%
Notice that the invariant above only constraints the hyper-state
relevant to the component 1.
%
Next, we represent the index sets of the format components as the
following two unions:
%
\vspace{-5pt}
%
{\small{
\begin{align*}
\set{
\angled{2, i, j}~\left|
\begin{array}{l} i \in [0, M) \\ j \in [0,N) \end{array}
\right.
} &= \biguplus_{i = 0}^{M - 1} \set{\angled{2, i, j}~|~j \in [0,N)}
\\
\set{\angled{3, j}~|~{j \in [0, N)}} &= 
\bigcup_{0}^{M - 1} \set{\angled{3, j} ~|~ {j \in [0, N)}}
\end{align*}
%
}}
%
%\vspace{-5pt}
%
\noindent
%
That is, while the first set has been split into $M$ disjoint
components, the second has been represented as a union of its own $M$
identical copies, as we will need it for \emph{each} of $M$ iterations
of the \code{for}-loop.
%
Choosing the invariant $\Ifor$ and the split leads to the following
proof obligation, after framing out all the unchanged components of
the state in the invariant:
%
\begin{equation}
\label{eq:csr3}
{\small{
\hspec{\!
\begin{array}{c}
  \Ans(1)+i \mapsto 0
  \\[2pt]
  \str~\ldots  
\end{array}
\!}    
\hmid{\!\!\!
  \begin{array}{c@{\ }c@{\ }l}
  1 &:& p(i)
  \\ [2pt]
  \angled{2, i, j}_{j \in [0, N)} &:&  \mathtt{csrij(m_{ind}, m_{val},} i, j)
  \\ [2pt]
  \angled{3, j}_{j \in [0, N)} &:& \mathtt{svi(x_{ind}, x_{val},} j) 
  \end{array}
\!}
\hspec{\!
\left.
\begin{array}{r}
- \\[2pt] \many{m} \\[2pt] \many{x}
\end{array}
\right|
\begin{array}{c}
{\Ans(1) + i} \mapsto \sum_j \many{m}(i,j)\many{x}(j) 
\\[2pt] \str \ldots
\end{array}
\!}
}}
\end{equation}
%
In the goal the implicitly universally quantified variable $i$ ranges
from $0$ up to $|\inds{m}| - 1$.
%
Since $i$ is fixed across all the programs in the second component
product, let us re-index it, simultaneously rewriting the call to
\code{csrij} with its definition (also notice a subtle change in using
$\many{m}$ in the postcondition):
%
%
\begin{equation}
\label{eq:csr4}
{\small{
\hspec{\!
\begin{array}{c}
  \Ans(1)+i \mapsto 0
  \\[2pt]
  \str~\ldots  
\end{array}
\!}    
\hmid{\!\!\!
  \begin{array}{c@{\ }c@{\ }l}
  1 &:& p(i)
  \\ [2pt]
  \angled{2, j}_{j \in [0, N)} &:&  \mathtt{svi(m_{ind}[i], m_{val}[i],} j)
  \\ [2pt]
  \angled{3, j}_{j \in [0, N)} &:& \mathtt{svi(x_{ind}, x_{val},} j) 
  \end{array}
\!}
\hspec{\!
\left.
\begin{array}{r}
- \\[2pt] \many{m} \\[2pt] \many{x}
\end{array}
\right|
\begin{array}{c}
{\Ans(1) + i} \mapsto \sum_j \many{m}(j)\many{x}(j) 
\\[2pt] \str \ldots
\end{array}
\!}
}}
\end{equation}
%
Progressing beyond line~3 of \code{spmspv} and allocating the
variable \code{iM} and \code{iX} leaves with the goal:
%
\begin{equation}
\label{eq:csr5}
{\small{
\!\!\!\!
\hspec{\! \! 
  \begin{array}{c}
    {\tt ans(1)}+i \mapsto 0 \str\!\! \\[2pt]
    \mcode{iX} \mapsto 0 \str
    \mcode{iM} \mapsto 0 \str \\[2pt]
    \ldots 
  \end{array}
\!\! \!}    
\hmid{\!\!\!
  \begin{array}{c@{\ }c@{\ }l}
  1 &:& \kw{while}\ (\dots) \{\dots\}
  \\ [2pt]
  \angled{2, j}_{j \in [0, N)} &:&  \mathtt{svi(m_{ind}[i], m_{val}[i],} j)
  \\ [2pt]
  \angled{3, j}_{j \in [0, N)} &:& \mathtt{svi(x_{ind}, x_{val},} j) 
  \end{array}
\!}
\hspec{\! \! \!
\left.
\begin{array}{r}
- \\[2pt] \many{m} \\[2pt] \many{x}
\end{array}
\right|
\begin{array}{c}
{\Ans(1) + i} \mapsto \sum_j \many{m}(j)\many{x}(j) 
\\[2pt] \str \ldots
\end{array}
\! \!\!}
}}
\end{equation}
First we consider a case when at least one of $\inds{x}$ or $\mind$ is empty, (say $\inds{x}$ then), $\kw{while}$-loop condition will be immediately false. More over using  \tname{Prod} and the following specification for \code{svi}
\noindent
\begin{equation*}
  % \label{eq:svi2}
  {\small{
  \hsll
  { \!\! 
    \arrl{\mcode{ind}}{\ind}\str 
    \arrl{\mcode{val}}{\val} \str
    \pure{j \notin \ind}
  \!\!\! }
  {
  \!\!
  \begin{array}{c@{\ }c@{\ }l}
  e :  \mcode{svi}(\mcode{ind}, \mcode{val}, j)
  \end{array}
  \!\!
  }
  {x}
  {\!\! 
  \begin{array}{l}
    \pure{x = 0}\str \ldots 
  \end{array}
  }}}
\end{equation*}
\noindent
which can be easily proven as a regular separation logic property, we conclude
\begin{equation}
  \label{eq:sviemp}
  {\small{
  \!\!\!\!
  \hspec{\! \! 
    \begin{array}{c}
      {\tt ans(1)}+i \mapsto 0 \str\!\! \\[2pt]
      \mcode{iX} \mapsto 0 \str
      \mcode{iM} \mapsto 0 \str \\[2pt]
      \ldots 
    \end{array}
  \!\! \!}    
  \hmid{\!\!\!
    \begin{array}{c@{\ }c@{\ }l}
    \angled{3, j}_{j \in [0, N)} &:& \mathtt{svi(x_{ind}, x_{val},} j) 
    \end{array}
  \!}
  \hspec{\! \! \!
  \left.
  \begin{array}{r}
   \many{x}
  \end{array}
  \right\vert
  \pure{\many{x} = \Zero}\str \ldots\ }
  }}
  \end{equation}
  Hence we can reduce~\eqref{eq:csr5}
  to 
\begin{equation}
\label{eq:csr5}
{\small{
\!\!\!\!
\hspec{\! \! 
  \begin{array}{c}
    {\tt ans(1)}+i \mapsto 0 \str\!\! \\[2pt]
    \mcode{iX} \mapsto 0 \str
    \mcode{iM} \mapsto 0 \str \\[2pt]
    \ldots 
  \end{array}
\!\! \!}    
\hmid{\!\!\!
  \begin{array}{c@{\ }c@{\ }l}
  \angled{3, j}_{j \in [0, N)} &:& \mathtt{svi(x_{ind}, x_{val},} j) 
  \end{array}
\!}
\hspec{\! \! \!
\left.
\begin{array}{r}
- \\[2pt] \many{m} \\[2pt] \many{x}
\end{array}
\right|
\begin{array}{c}
{\Ans(1) + i} \mapsto 0
\\[2pt] \str \ldots
\end{array}
\! \!\!}
}}
\end{equation}
Which immediately follows form \code{svi} termination (it is a \code{for}-loop under the hood).
%
To proceed in the case when both $\inds{x}$ and $\inds{m}[i]$ are both non-empty, let us make an important observation.
%
Remember that both arrays $\inds{m}[i]$ and $\inds{x}$ contain indices
of non-zero elements of the corresponding dense vectors. 
%
Therefore any elements of those vectors positioned at indices larger
than $\St = \min(\max(\inds{m}[i]), \max(\inds{x}))$ will \emph{not}
contribute to the sum stored in \code{ans(1)} due to either being
zero or being multiplied by zero.
%
This fact can be phrased as the following hyper-safety triple:
%
\begin{equation}
\label{eq:csr6}
  {\small{
  \hsll
  { \!\! \dots \begin{array}{l}\phantom{a}\\[2pt]\phantom{a}\end{array} \!\! \!\! \!\! \!\! \!\! \!\!\! }
  {
  \!\!
  \begin{array}{c@{\ }c@{\ }l}
  \angled{2,j}_{\St < j < N} &:&  \mathtt{svi(m_{ind}[i], m_{val}[i],} j)
  \\ [2pt]
  \angled{3,j}_{\St < j < N} &:& \mathtt{svi(x_{ind}, x_{val},} j) 
  \end{array}
  \!\!
  }
  {\many{m} \\ \many{x}}
  {\!\!  \pure{\forall j > \St,\ \many{m}(j)\many{x}(j) = 0} \!\!}  
  }}
\end{equation}
%
Using the rule \rulename{SeqU} we can, therefore,
reduce~\eqref{eq:csr5} to the following goal:
%
\begin{equation}
\label{eq:csr7}
{\small{
\!\!\!\!
\hspec{\! \! 
  \begin{array}{c}
    {\tt ans(1)}+i \mapsto 0 \str\!\! \\[2pt]
    \mcode{iX} \mapsto 0 \str
    \mcode{iM} \mapsto 0 \str \\[2pt]
    \ldots 
  \end{array}
\!\! \!}    
\hmid{\!\!\!
  \begin{array}{l}
  \phantom{a}~1 : \kw{while}\ \mcode{(cond(iM,iX))} \set{\ldots}
  \\ [2pt]
  \angled{2,j}_{j \leq \St} :  \mathtt{svi(m_{ind}[i], m_{val}[i],} j)
  \\ [2pt]
  \angled{3,j}_{j \leq \St} : \mathtt{svi(x_{ind}, x_{val},} j) 
  \end{array}
\!}
\hspec{\! \! \!
\left.
\begin{array}{r}
- \\[2pt] \many{m} \\[2pt] \many{x}
\end{array}
\right|
\begin{array}{c}
{\Ans(1) + i} \mapsto \sum_j \many{m}(j)\many{x}(j) 
\\[2pt] \str \ldots
\end{array}
\! \!\!}
}}
\end{equation}
%
where \code{cond(iM, iX)} abbreviates the actual condition of the
\code{while}-loop.

\paragraph{Step 2: Verifying the \code{while}-loop}
%
We are going to use the general \rulename{While} rule to verify the
goal~\eqref{eq:csr7}.
%
Recall that this rule in \logic provides access
to the \emph{counting} aspect of a \code{while}-loop. 
%
This is thanks to the second parameter~$s$ of its invariant of the
shape $\Iwl(b, s, \many{v})$ that ``keeps track'' of the number of
(format-related) ``auxiliary'' program components used to verify the
previous loop iterations.
%
The first invariant parameter, $b$, keeps the status of the loop
condition, while the last, $\many{v}$ accumulates the hyper-value
containing the results of the auxiliary programs executed in alignment
with the past iterations.
%
To make use of the rule for our example, we choose the following invariant:
%
\begin{equation} 
\label{eq:csr8}
  \small{
  \begin{array}{r@{\ }c@{\ }l@{\ }l}
    \Iwl(b, s,\many{m}\many{x}) & \eqdef 
   & \exists \Imm, \Ixx, & \mcode{iM} \mapsto\Imm \leq |\inds{m}[i]| \str \mcode{iX}
                           \mapsto \Ixx \leq |\inds{x}| \str \mcode{cond}(\Imm, \Ixx) \Leftrightarrow b \str \\[2pt]
   &&& \pure{\min(x_0, m_0) = s} \str\\[2pt]
   &&& \Ans(1) + i \mapsto \sum_{j < s} \many{m}(j)\many{x}(j) \str \\[2pt]
   &&& \pure{x_0 < m_0 \Rightarrow \forall m \in \inds{m}[i],\ m < m_0 \Rightarrow m < x_0} \str \\[2pt]
   &&& \pure{m_0 < x_0 \Rightarrow \forall x \in \inds{x},\ x < x_0 \Rightarrow x < m_0}
  \end{array}}
\end{equation}
Where with $x_0$ we denote $\inds{x}[\Ixx]$ if $\Ixx < \code{length}(\inds{x})$ and $\max(\inds{x}) + 1$ otherwise. Same for $m_0$.

The first line of the invariant simply gives names to the values
stored in the vector counters ($\Imm$ and $\Ixx$) and relates their
values to the loop condition $b$.
%
The second line is the most subtle:
%
it captures the overall ``progress'' through the dense pair of the
dense vectors being multiplied by storing the minium of $\inds{x}[ix]$
and $\inds{m}[i][im]$ in the variable $s$, which according to the rule
premises, also counts the number of auxiliary programs ``dispatched''
by that time. 
%
This assertion is crucial for determine the \emph{lower boundary} for
the index~$j$ determining which components to include for alignment
with the current loop iteration and what portion of the product of the
two vectors has been already accumulated in the element $\Ans(1) + i$
of the result (the last assertion in \eqref{eq:csr8}).

Finally last two lines ensure that $x_0$ and $m_0$ are in some sense closest values of $\inds{x}$ and $\inds{m}[i]$. For instance if $x_0 < m_0$, $m_0$ is the smallest value of $\inds{m}[i]$ which is still greater that $x_0$.

We assume our index set division to be 
\noindent
\begin{equation*}
  \small{
  \{\angled{2,j}\ |\ j \in [s, \St+1) \} \cup \{\angled{3,j}\ |\ j \in [s, \St+1) \} = \bigcup_{j=0}^{\St+1 -1} \{ \angled{2,j}, \angled{3,j} \}}
\end{equation*}

Note that $\Iwl(s, \False, \many{v})$ implies that
$\mcode{cond}(\Ixx, \Imm)$ is false, hence either $\Ixx \geq |\xind|$
or $\Imm \geq |\mind|$. However $\Iwl$ ensures $\Ixx \geq |\ind{x}|$
and $\Imm \leq |\ind{m}[i]|$. So in that case one of $\Imm$ and $\Ixx$
equals to the size of the correspondent array, hence $s = \St + 1$.
Which is exactly our upper bound ($M$ in \tname{While}).

Abbreviating the body of the \code{while}-loop as~$q$ and applying the
rule \rulename{While} gives us the following:
%
\begin{equation}
\label{eq:csr9}
  {\small{
  \hsll
  { \!\! 
  \Iwl(s, \True, \many{m}\many{x}) \!\!\! }
  {
  \!\!
  \begin{array}{c@{\ }c@{\ }l}
  1 &:& q; \kw{while}(\mcode{cond(iM, iX)})~\set{q}
  \\ [2pt]
  \angled{2,j}_{s \leq j \leq \St} &:&  \mathtt{svi(\inds{m}[i], \vals{m}[i],} j)
  \\ [2pt]
  \angled{3,j}_{s \leq j \leq \St} &:& \mathtt{svi(\inds{x}, \vals{x},} j) 
  \end{array}
  \!\!
  }
  {- \\ \many{m} \\ \many{x}}
  {\!\! 
  {\Iwl(\False, \St+1, \many{m}\many{x})\!\!}  
  }}}
\end{equation}
%
Since the body of the loop is an \code{if}-statement, the rest of the
proof proceeds by the case analysis.

In first case, $\xind[ix] = \mind[im]$. Let us define
$s' \eqdef \min(\xind[ix+1],\mind[im+1])$, which should be a new
value of the ``auxiliary program counter'' $s$ after this iteration. 
%
This brings us to
%
\begin{equation}
\label{eq:csr10}
{\small{
    \hsll
    { \!\! 
      \Iwl(\True, s, \many{m}\many{x}) \!\!\! }
    {
      \!\!
      \begin{array}{c@{\ }c@{\ }l}
        1 &:& q
        \\ [2pt]
        \angled{2,j}_{j \in [s,s')} &:&  \mathtt{svi(\inds{m}[i], \vals{m}[i],} j)
        \\ [2pt]
        \angled{3,j}_{j \in [s,s')} &:& \mathtt{svi(\inds{x}, \vals{x},} j) 
      \end{array}
      \!\!
    }
    {- \\ \many{m}' \\ \many{x}'}
    {\!\! 
    {\Iwl(b', s', \many{m}'\many{m}\many{x}'\many{x})\!\!}  
    }}}
\end{equation}
%
The post-condition of~\eqref{eq:csr10} will therefore serve as a
precondition to the induction hypothesis about the next iteration of
the \code{while}-loop from the premise of the \rulename{While} rule,
%
Furthermore, the statement of~\eqref{eq:csr10} means that the current
iteration of the body of the loop, will process all elements $x[i]$
and $m[i][j]$ in a pair-wise fashion for all~$j$ such that
$s \leq j < s'$.
%
To prove this goal, let us execute $q$ to completion, updating the
values of \code{ans}, \code{iM}, and \code{iX}, resulting in the
following goal, where $y$ binds the accumulated sum
$\sum_{j < s} \many{m}(j)\many{x}(j)$ and all irrelevant parts of the
invariant are omitted:
%
\begin{equation}
\label{eq:csr11}
{\small{
    \hsll
    { \!\! 
      \Ans(1) + i \mapsto
      \\[2pt] 
      \phantom{aaaa} y + \xind[\Ixx]\mind[\Imm]
      \\[2pt] 
      \str \ldots \!\!\! }
    {
    \!\!
    \begin{array}{c}
    1 : \mcode{skip}  
    \\ [2pt]
    \angled{2,j}_{j \in [s,s')} :  \mathtt{svi(\dots})
    \\ [2pt]
    \angled{3,j}_{j \in [s,s')} : \mathtt{svi(\dots}) 
    \end{array}
    \!\!
    }
    {- \\ \many{m}' \\ \many{x}'}
    {\!\! 
    \begin{array}{l}
      \Ans(1) + i \mapsto 
      \\[2pt]
      \phantom{aaaa} y + \sum_{j = s}^{s'-1} \many{m}'(j)\many{x}'(j) 
      \\[2pt]
       \str \ldots
    \end{array}
    
    }}}
\end{equation}
%
We prove this goal by showing that $\xval[\Ixx]$ and $\mval[\Imm]$ are
the only \emph{simultaneously} non-zero values of $\many{x}'$ and
$\many{m'}$.
%
Recall that $s = \xind[\Ixx] = \mind[i][\Imm]$ and
$s' = \min(\xind[\Ixx+1], \mind[i][\Imm+1])$, which excludes both
$\xind[\Ixx+1]$ and $\mind[i][\Imm+1]$ from the domains of $\many{x}'$
and $\many{m'}$.

This fact can be derived from the following two complementary
specifications of \code{svi}:
%
\begin{equation}
\label{eq:svi1}
{\small{
    \hsll
    { \!\!\!
      \arrl{\mcode{ind}}{\ind}\str 
      \arrl{\mcode{val}}{\val} \str
        \pure{j = \ind[i]}
    \!\!\! }
    {
    \!\!
    \begin{array}{c@{\ }c@{\ }l}
    e :  \mcode{svi}(\mcode{ind}, \mcode{val}, j)
    \end{array}
    \!\!
    }
    {x}
    {\!\! 
      \pure{x = \val[i]}\str \ldots
    \!
    }}}
  \end{equation}
  \noindent
  \begin{equation}
    \label{eq:svi2}
    {\small{
    \hsll
    { \!\! 
      \arrl{\mcode{ind}}{\ind}\str 
      \arrl{\mcode{val}}{\val} \str
      \pure{j \notin \ind}
    \!\!\! }
    {
    \!\!
    \begin{array}{c@{\ }c@{\ }l}
    e :  \mcode{svi}(\mcode{ind}, \mcode{val}, j)
    \end{array}
    \!\!
    }
    {x}
    {\!\! 
    \begin{array}{l}
      \pure{x = 0}\str \ldots 
    \end{array}
    }}}
\end{equation}
%
The second specification can be used for any $j$, such that
$s < j < s'$, which implies that it's neither in $\xind$ nor in
$\mind[i]$.
%
Both~\eqref{eq:svi1} and~\eqref{eq:svi2} can be derived in unary
separation logic.

Let't consider other parts of the invariant, that we have to prove:
\begin{equation*}
  \small{
  \begin{array}{l}
  \mcode{iM} \mapsto\Imm+1 \leq |\inds{m}[i]| \str \mcode{iX}
                           \mapsto \Ixx+1 \leq |\inds{x}| \str \\[2pt]
   \pure{\min(\inds{x}[\Ixx + 1], \inds{im}[\Imm+1]) = s'} \str\\[2pt]
   \pure{x_0 < m_0 \Rightarrow \forall m \in \inds{m}[i],\ m < m_0 \Rightarrow m < x_0} \str \\[2pt]
   \pure{m_0 < x_0 \Rightarrow \forall x \in \inds{x},\ x < x_0 \Rightarrow x < m_0}
  \end{array}}
\end{equation*}
\noindent
Where with $x_0$ and $m_0$ we denote $\inds{x}[\Ixx+1]$ and $\mind[\Imm+1]$. First two lines are trivial. Let's consider last two lines. As they are symmetric we consider only first of them. Assume $\inds{x}[\Ixx+1] < \inds{m}[i][\Imm+1]$ and $ m \in \inds{m}[i]$ such that $m < \inds{m}[i][\Imm+1]$. Because of the fact that $\inds{m}[i]$ is sorted we derive that  $m \leq \inds{m}[i][\Imm]$. The fact that $m < x_0$ follow from 
\noindent
\[ \small{m \leq \inds{m}[i][im] = \inds{x}[ix] < x_0}\]

%%%%%%%%%%%%%%%%%

In the second case for~\eqref{eq:csr9}, $\xind[\Ixx] < \mind[\Imm]$,
which makes the goal~\eqref{eq:csr10} true for
$s' = \min(\xind[\Ixx+1],\mind[\Imm])$. 
%
To prove this goal, let us execute $q$ to completion, updating the
values of \code{ans}, \code{iM}, and \code{iX}, resulting in the
following goal, where $y$ binds the accumulated sum
$\sum_{j < s} \many{m}(j)\many{x}(j)$ and all irrelevant parts of the
invariant are omitted:
%
\begin{equation}
\label{eq:csr11}
{\small{
    \hsll
    { \!\! 
      \Ans(1) + i \mapsto
      \\[2pt] 
      \phantom{aaaa} y
      \\[2pt] 
      \str \ldots \!\!\! }
    {
    \!\!
    \begin{array}{c}
    1 : \mcode{skip}  
    \\ [2pt]
    \angled{2,j}_{j \in [s,s')} :  \mathtt{svi(\dots})
    \\ [2pt]
    \angled{3,j}_{j \in [s,s')} : \mathtt{svi(\dots}) 
    \end{array}
    \!\!
    }
    {- \\ \many{m}' \\ \many{x}'}
    {\!\! 
    \begin{array}{l}
      \Ans(1) + i \mapsto 
      \\[2pt]
      \phantom{aaaa} y + \sum_{j = s}^{s'-1} \many{m}'(j)\many{x}'(j) 
      \\[2pt]
       \str \ldots
    \end{array}
    
    }}}
\end{equation}
%
We prove this goal by showing that there no \emph{simultaneously} non-zero values of $\xval[\Ixx]$ and $\mval[\Imm]$ between $s$ and $s'$.
%
Recall that $s = \xind[\Ixx] < \mind[\Imm]$ and
$s' = \min(\xind[\Ixx+1], \mind[\Imm])$, which excludes
$\xind[\Ixx+1]$. So the only non-zero value of $\xind$ there is $\xind[\Ixx]$. Assume that there is $m \in \mind$ such that $m = \xind[\Ixx]$. In that case $m < \mind[\Imm]$. And because of our invariant it should be less then $\xind[\Ixx]$. So there is no such value $m$, thus all values of $\many{m'x'}$ are zeros.

Now we have to prove

\begin{equation*}
  \small{
  \begin{array}{l}
  \mcode{iM} \mapsto\Imm \leq |\inds{m}[i]| \str \mcode{iX}
                           \mapsto \Ixx+1 \leq |\inds{x}| \str \\[2pt]
   \pure{\min(\inds{x}[\Ixx + 1], \inds{im}[\Imm]) = s'} \str\\[2pt]
   \pure{x_0 < m_0 \Rightarrow \forall m \in \inds{m}[i],\ m < m_0 \Rightarrow m < x_0} \str \\[2pt]
   \pure{m_0 < x_0 \Rightarrow \forall x \in \inds{x},\ x < x_0 \Rightarrow x < m_0}
  \end{array}}
\end{equation*}
\noindent
Where with $x_0$ and $m_0$ we denote $\inds{x}[\Ixx+1]$ and $\mind[\Imm]$. First two lines are trivial. Let's consider last two lines.

Assume $\inds{x}[\Ixx+1] < \mind[\Imm]$ and $ m \in \inds{m}[i]$ such that $m < \inds{m}[i][\Imm]$. We know that $\xind[\Ixx] < \inds{x}[\Ixx+1]$, because $\xind$ is sorted. Hence $\xind[\Ixx] < \mind[\Imm]$. But our invariant holds for $\Imm$ and $\Ixx$, hence by its last line we conclude that $m < \xind[\Ixx]$.

Finally consider the the case when $\mind[\Imm] < \inds{x}[\Ixx+1]$, and  $x \in\xind$ such that $x < \xind[\Ixx+1]$. The last fact due to sortedness of $\xind$ implies that $x \leq \xind[\Ixx]$. But we are considering the case where $\xind[\Ixx] < \mind[\Imm]$. Hence $x < \mind[\Imm]$.

%%%%%%%%%%%%
The third case when $\xind[\Ixx] > \mind[\Imm]$ is analogous to the second one.





% Firладнt note that if at least one of $x_{ind}$ or $m_{ind}[i]$ is empty, then $st$ would be the minium of maximums of empty array. Which id by our convention is -1. Hence two of index sets $\angled{2,j}_{j \leq st}$ and $\angled{3,j}_{j \leq st}$ are empty, and the while loop will never be executed. So the triple holds trivially.

% Thus we assume that both of $x_{ind}$ and $m_{ind}[i]$ are not empty. Our full invariant is

% \begin{equation*} {
%   \small{
%     I(b, s,\many{m},\many{x}) \eqdef 
% \exists im\, ix,\ 
%   \begin{array}{l}
%   iM \mapsto im \str iX\mapsto ix \str \\[2pt]
%   \pure{{\tt min}(x_0, m_0) = s} \str\\[2pt]
%   {\tt ans} + i \mapsto \sum_{j < s} \many{m}(i,j)\many{x}(j) \str \\[2pt]
%   {\tt cond}(im,ix) \leftrightarrow b \str \\[2pt]
%   \pure{x_0 < m_0 \Rightarrow \forall m \in m_{ind}[i],\ m < m_0 \Rightarrow m < x_0} \\[2pt]
%   \pure{m_0 < x_0 \Rightarrow \forall x \in x_{ind},\ x < x_0 \Rightarrow x < m_0}
%   \end{array}}}
% \end{equation*}

% Where by $x_0$ and $m_0$ we denote $x_{ind}[ix]$ and $m_{ind}[i][im]$. Note that in our convention, for non-empty $s$, if $i \geq |s|$, $s[i]$ is define as the last value of $s$ plus one.

% Last two conjuncts denote that $x_0$ and $m_0$ are in some sense closest values of $x_{ind}$ and $m_{ind}[i]$. For instance if $x_0 < m_0$, then $m_0$ is the smallest value of $m_{ind}[i]$ which is still greater that $x_0$.

% We use the following division of our index set 

% \[\small \angled{2,j}_{j \leq st} \cup \angled{3,j}_{j \leq st} = \biguplus_{j = 0}^{st} \{ \angled{2,j}, \angled{3,j} \} \]

% Note that $I({\tt false}, s, \many{m},\many{x})$ implies that condition is false. Hence at least of one $im$ or $ix$ would be out of its bounds. Because of our convention one of $x_0$ or $m_0$ would be maximal element of the correspondent array plus one. Hence $s = st + 1$, and the post condition holds. 

% Now, denoting the loop body with $p$, we have to show 

% \begin{equation}
%   \label{eq:goal}
%   % \label{eq:rlprod2}
%   {\small{
%   \hsll
%   { \!\! 
%   I({\tt true}, s, \many{m},\many{x}) \!\!\! }
%   {
%   \!\!
%   \begin{array}{c@{\ }c@{\ }l}
%   1 &:& p
%   \\ [2pt]
%   \angled{2,j}_{j \geq s} &:&  \mathtt{svi(m_{ind}[i], m_{val}[i],} j)
%   \\ [2pt]
%   \angled{3,j}_{j \geq s} &:& \mathtt{svi(x_{ind}, x_{val},} j) 
%   \end{array}
%   \!\!
%   }
%   {\_ \\ \many{m} \\ \many{x}}
%   {\!\! 
%   {I(st, {\tt false}, \many{m}, \many{x})\!\!}  
%   }}}
% \end{equation}

% Using 

% \begin{equation}
%   \label{eq:ih}
%   % \label{eq:rlprod2}
%   {\small{
%   \hsll
%   { \!\! 
%   I({\tt true}, s', \many{m},\many{x}) \!\!\! }
%   {
%   \!\!
%   \begin{array}{c@{\ }c@{\ }l}
%   1 &:& p; w
%   \\ [2pt]
%   \angled{2,j}_{j \geq s'} &:&  \mathtt{svi(m_{ind}[i], m_{val}[i],} j)
%   \\ [2pt]
%   \angled{3,j}_{j \geq s'} &:& \mathtt{svi(x_{ind}, x_{val},} j) 
%   \end{array}
%   \!\!
%   }
%   {\_ \\ \many{m} \\ \many{x}}
%   {\!\! 
%   {I(st, {\tt false}, \many{m}, \many{x})\!\!}  
%   }}}
% \end{equation}

% For some $s'$ greater then $s$.

% Let $im$ and $ix$ be two current values of $iM$ and $iX$. We consider 2 cases: $x_{ind}[ix] = m_{ind}[im]$ and $x_{ind}[ix] > m_{ind}[iM]$. Third case when $x_{ind}[ix] < m_{ind}[im]$ is analogous to the second one.

% \begin{enumerate}
%   \item Let $x_{ind}[ix] = m_{ind}[im]$. Denote $s'$ to be ${\tt min}(x_{ind}[ix+1], m_{ind}[im+1])$. We show 
%   \begin{equation}
%     \label{eq:step1}
%     {\small{
%     \hsll
%     { \!\! 
%     I({\tt true}, s, \many{m},\many{x}) \!\!\! }
%     {
%     \!\!
%     \begin{array}{c@{\ }c@{\ }l}
%     1 &:& p
%     \\ [2pt]
%     \angled{2,j}_{j \in [s,s')} &:&  \mathtt{svi(m_{ind}[i], m_{val}[i],} j)
%     \\ [2pt]
%     \angled{3,j}_{j \in [s,s')} &:& \mathtt{svi(x_{ind}, x_{val},} j) 
%     \end{array}
%     \!\!
%     }
%     {\_ \\ \many{m_1} \\ \many{x_1}}
%     {\!\! 
%     {I(b', s', \many{m_1m}, \many{x_1x})\!\!}  
%     }}}
%   \end{equation}
%   After we execute the loop body our pre-condition will become 
%   \[\small 
%     \begin{array}{l} 
%        iM \mapsto im+1 \str iX \mapsto ix+1 \str \\[2pt]
%        {\tt ans}+i \mapsto \dots + x_{val}[ix]m_{val}[im] 
%     \end{array}\]
%   We have to show that $\sum_{j \in [s,s')} \many{m_1}(i,j)\many{x}(j)$ equals to $x_{val}[ix]m_{val}[im]$, where $\many{m_1}$ and $\many{x_1}$ are results of correspondent $\tt svi$s. Which is trivial because the only values of $x_{ind}$ and $m_{ind}[i]$ in the interval $[s, s')$ are  $x_{ind}[ix]$ and $m_{ind}[im]$. 

%   Now are left to show 
%   \begin{equation*}
%     % \label{eq:step1}
%     \small{
%      \begin{array}{l}
%     \pure{x_0 < m_0 \Rightarrow \forall m \in m_{ind}[i],\ m < m_0 \Rightarrow m < x_0} \\[2pt]
%     \pure{m_0 < x_0 \Rightarrow \forall x \in x_{ind},\ x < x_0 \Rightarrow x < m_0}
%     \end{array}}
%   \end{equation*}
%   Where by $x_0$ and $m_0$ we denote $x_{ind}[ix+1]$ and $m_{ind}[i][im+1]$. This two facts are symmetric so we consider only the case when $x_0 < m_0$.
%   Assume $m < m_0$. Then, because of the sortedness of $m_{ind}[i]$, we conclude $m \leq m_{ind}[i][im]$. We reach the conclusion by noticing:
%   \[ m \leq m_{ind}[i][im] = x_{ind}[ix] < x_0\]
%   \item Let $x_{ind}[ix] > m_{ind}[im]$. Because of the invariant we conclude 
%   \begin{equation*} 
%     \label{eq:aux}
%     \forall x \in x_{ind}, x \geq x_{ind}[ix] \lor x < m_{ind}[i][im] 
%   \end{equation*}
%    Denote $s'$ to be ${\tt min}(x_{ind}[ix], m_{ind}[im+1])$. We show 
%   \begin{equation}
%     \label{eq:step2}
%     {\small{
%     \hsll
%     { \!\! 
%     I({\tt true}, s, \many{m},\many{x}) \!\!\! }
%     {
%     \!\!
%     \begin{array}{c@{\ }c@{\ }l}
%     1 &:& p
%     \\ [2pt]
%     \angled{2,j}_{j \in [s,s')} &:&  \mathtt{svi(m_{ind}[i], m_{val}[i],} j)
%     \\ [2pt]
%     \angled{3,j}_{j \in [s,s')} &:& \mathtt{svi(x_{ind}, x_{val},} j) 
%     \end{array}
%     \!\!
%     }
%     {\_ \\ \many{m_1} \\ \many{x_1}}
%     {\!\! 
%     {I(b', s', \many{m_1m}, \many{x_1x})\!\!}  
%     }}}
%   \end{equation}
%   After we execute the loop body our pre-condition will become 
%   \[\small 
%     \begin{array}{l} 
%        iM \mapsto im+1 \str iX \mapsto ix \str \\[2pt]
%        {\tt ans}+i \mapsto \sum_{j < s} \dots
%     \end{array}\]
%   We have to show that $\sum_{j \in [s,s')} \many{m_1}(i,j)\many{x}(j)$ equals to 0, where $\many{m_1}$ and $\many{x_1}$ are results of correspondent $\tt svi$s. The only value of $m_{ind}[i]$ in $[s,s')$ is $m_{ind}[i][im]$. So 
%   \noindent
%   \[\sum_{j \in [s,s')} \many{m_1}(i,j)\many{x}(j) = \many{m_1}(i,m_{ind}[i][im]) \many{x_1}(m_{ind}[i][im]) \]
%   \noindent
%   However $m_{ind}[i][im]$ doesn't satisfy any disjuncts in~\eqref{eq:aux}. Hence $m_{ind}[i][im] \notin x_{ind}$. Hence $\many{x_1}(m_{ind}[i][im]) = 0$. And the summation is indeed 0.

%   Now are left to show 
%   \begin{equation*}
%     \small{
%      \begin{array}{l}
%     \pure{x_0 < m_0 \Rightarrow \forall m \in m_{ind}[i],\ m < m_0 \Rightarrow m < x_0} \\[2pt]
%     \pure{m_0 < x_0 \Rightarrow \forall x \in x_{ind},\ x < x_0 \Rightarrow x < m_0}
%     \end{array}}
%   \end{equation*}
%   Where by $x_0$ and $m_0$ we denote $x_{ind}[ix]$ and $m_{ind}[i][im+1]$. Consider both cases
%   \begin{enumerate}
%     \item Let $x_{ind}[ix] < m_{ind}[i][im+1]$, and $m <  m_{ind}[i][im+1]$. Because of the sortedness of $m_{ind}[i]$, we have $m \leq m_{ind}[i][im]$. We reach the conclusion by noticing:
%     \[ m \leq m_{ind}[i][im] < x_{ind}[ix] < x_0\]
%     \item  Let $m_{ind}[i][im+1] < x_{ind}[ix]$ and $x <  x_{ind}[ix]$. Because of the invariant we conclude $x < m_{ind}[i][im]$. So as $m_{ind}[i]$ is sorted, $x < m_{ind}[i][im+1]$
%   \end{enumerate}
% \end{enumerate}
% \noindent
% Finally, combining~\eqref{eq:step1} in the first case and~\eqref{eq:step2} with~\eqref{eq:ih} we obtain~\eqref{eq:goal}.





==> case-study-coq.tex <==

\section{A Commentary for the Mechanised Proof of RL Summation}
\label{sec:case-study-coq}

We have mechanised the case study in Sections 1 and 2 of the
manuscript in Coq. Our mechanised proof mainly follows the proof
outline of Section 2, and it is modular in the sense that each
important intermediate proof step, represented as hyper-triple here,
as a lemma.

We have attached a navigation guide of our mechanisation in the
accompanying Coq project directory for illustrating the correspondence
between the results in the paper and the lemmas proved in Coq. Here we
only provide a general, conceptual explanation of the differences
between our mechanised proof and the textual proof.

Some technical details that are present in the Coq proof, but not in
the paper:

\begin{itemize}
\item An array not only contains a sequence of memory blocks, but also
  includes a header that stores its length information. In the
  semantics, applying the length operator on the header will return
  its content.
%
\item Functions are written in a form similar to that of an
  intermediate language resembling three-address code, in order to fit
  the operational semantics.
\end{itemize}

\noindent
%
Some changes in the Coq formalisation that are made to reduce the
reasoning burden: 

\begin{itemize}
%
\item The lengths of arrays $\xind, \xval$ are hard-coded by assuming
  them as existing variables. In other words, they are not obtained
  via the length operator. Similarly for their contents. 
%
\item The
  local variables (\eg, \code{i} in \code{rlsum}) are
  freed before the function returns. This change is made since
  reasoning about $\top$ would be complicated when applying the
  \textsc{Merge} rule. 
%
\end{itemize}


==> case.tex <==

\section{Case Study: Sparse Tensor Multiplication}
\label{sec:case}

To showcase \logic in its full glory, we turn our attention to a class
of algorithms that manipulate on \emph{sparse} data representations.
%
% and, in particular on sparse tensors that are in their simplest form
% just vectors and matrices
%
The program we verify in this section is a multiplication of a sparse
matrix by a sparse array---arguably one of the most common operations
used extensively in applications such as image processing, scientific
simulations, and neural network training.

\begin{figure}[t]
\begin{tabular}{cc}
\begin{tabular}{c}
\begin{subfigure}{0.45\textwidth}
\begin{minted}[numbers=left, xleftmargin=2.0ex, numbersep=6pt, escapeinside=@@, fontsize=\footnotesize]{python3}
def svi(x_ind, x_val, i):
  x = 0
  for j in range(0, length(x_ind)):
    if i = x_ind[j]:
      x = x_val[j]
  return x
    \end{minted}
    \caption{Sparse Vector (SV) format}
    \label{fig:sv}    
\end{subfigure}    
\\[20pt]
\begin{subfigure}{0.45\textwidth}
\begin{minted}[numbers=left, xleftmargin=2.0ex, numbersep=6pt, escapeinside=@@, fontsize=\footnotesize]{python3}
def csrij(m_ind, m_val, i, j):
  svi(m_ind[i], m_val[i], j)
\end{minted}
\caption{Compressed Sparse Row (CSR)}
\label{fig:csr}  
\end{subfigure}    
\end{tabular}
&
\begin{minipage}{0.45\linewidth}
\begin{subfigure}{1.0\linewidth}
\vspace{-10pt}
\begin{tabular}{c}
\includegraphics[width=0.45\linewidth]{figures/sv.pdf}    
\\
\vspace{-5pt}
\includegraphics[width=0.80\linewidth]{figures/csr.pdf}      
\end{tabular}
\caption{SV and CSR pictographically}
\label{fig:csr-pics}                  
\end{subfigure}
\end{minipage}
\end{tabular}
% \setlength{\abovecaptionskip}{5pt}
% \setlength{\belowcaptionskip}{-10pt}
\caption{Sparse Vector and Compressed Sparse Row formats}
\label{fig:csr-formats}  
\end{figure}

\subsection{Encoding Sparsity}
%
Multiple formats exist to represent sparse tensors compactly by
storing only their non-zero elements and their positions.
%
\autoref{fig:sv} and \autoref{fig:csr} provide two of the most common
formats for representing sparse 1-dimensional vectors and
2-dimensional matrices. 
%
The sparse vector (SV) format is represented by the decoding procedure
\code{svi} that restores a dense representation \code{x} from two
same-length arrays that encode the sparsity information: \code{x_ind}
storing indices of non-zero elements, and \code{x_val} storing their
values (\autoref{fig:sv}).
%
The popular Compressed Sparse Row (CSR) format is used to store sparse
matrices. CSR relies on SV to compress each row in the matrix, and
stores the resulting arrays \code{ind} and \code{val} contiguously.
Normally, a dense array \code{ptr} would be used to store the
locations of the boundaries between rows. In this work, for
simplicity, we instead store \code{ind} and \code{val} as dense arrays
of dense arrays.
%
The corresponding decoding procedure \code{csrij} (\autoref{fig:csr}),
which uses \code{svi} as its subroutine, takes two 2-dimensional
arrays representing a matrix~$m$: \code{m_ind} whose element
\code{m_ind[i]} for each \code{i} is an array of indices of the
\code{i}\ith compressed row of~$m$, and \code{m_val[i]} that stores
the non-zero values of~$m$'s \code{i}\ith row.

\subsection{Sparse Matrix/Vector Multiplication}
%

\begin{wrapfigure}[13]{r}{0.51\textwidth}
\vspace{-12pt}
\begin{minted}[numbers=left, xleftmargin=2.5ex, numbersep=6pt, escapeinside=@@, fontsize=\footnotesize]{python3}
def spmspv(m_ind, m_val, x_ind, x_val, ans)
  for i in range(0,length(m_ind)):
    iM, iX = 0, 0
    while (iM < length(m_ind[i])) && 
          (iX < length(x_ind)):
      if m_ind[i][iM] = x_ind[iX]:
        ans[i] += m_val[i][iM] * x_val[iX]
        iM++; iX++
      else if m_ind[i][iM] < x_ind[iX]:
        iM++
      else if x_ind[iX] < m_ind[i][iM]:
        iX++
\end{minted}
\setlength{\abovecaptionskip}{10pt}  
\caption{Sparse matrix/vector product (SpMSpV)}
\label{fig:smpv}
\end{wrapfigure}    
%
The procedure \code{spmspv} in \autoref{fig:smpv} shows the code of
the SpMSpV procedure that computes a result of multiplying a
CSR-encoded matrix~$m$ represented by the arrays \code{m_ind} and
\code{m_val} and of a sparse vector~$x$, encoded via \code{x_ind} and
\code{x_val}, filling a dense array \code{ans}, which is passed as the
last parameter.
%
Such code can be produced by one of the several existing compilers for
sparse and structured data, such as TACO~\cite{KjolstadKCLA17} or
\tname{Finch}~\cite{AhrensDKA23}.
%
A curious aspect of the SpMSpV implementation in \autoref{fig:smpv} is
that it efficiently \emph{co-iterates} on a combination of two sparse
vectors, \ie a row of the matrix~$m$ and the vector~$x$, via the loop
\code{while}-loop at lines 4-11.
%
Intuitively, it does so by maintaining the positions in the
corresponding vectors via variables \code{iM} and \code{iX}, advancing
them in a way so that the result stored in \code{ans[i]} is changed
only when indices of non-zero elements in the two vectors coincide
(line~6), skipping through any other cases.

To specify the result of \code{spmspv} compactly, let us introduce
some convenient notation.
%
First, we will use $\Zero$ to denote a 0-filled vector of a suitable
size evident from the context.
%
Second, we will abbreviate the joint assertion about all required
arrays across multiple components, which are not being modified,
simply as $\arrs$:
%
\begin{equation*}
{\small{
\arrs \eqdef \arr{\tinds{m}(\cdot)}{\inds{m}} \str
\arr{\tvals{m}(\cdot)}{\vals{m}} \str \arr{\tinds{x}(\cdot)}{\inds{x}}
\str \arr{\tvals{x}(\cdot)}{\vals{x}}
}}  
\end{equation*}
%
The desired specification is encoded by the following hypersafety triple:
%
\begin{equation}
\label{eq:csr1}
{\small{
\hspec{\!\!\!
\begin{array}{c}
  \arr{ans(1)}{\Zero} 
  \\[2pt]
  \str~\arrs  
\end{array}
\!\!\!}    
\hmid{\!\!\!
  \begin{array}{c@{\ }c@{\ }l}
  1 : \mathtt{spmspv(m_{ind}, m_{val}, x_{ind}, x_{val}, ans)} 
  \\ [2pt]
  \angled{2, i, j}_{\!\!\!\!\tiny
    \begin{array}{l} i \in [0, M) \\ j \in [0,N) \end{array}} :  \mathtt{csrij(m_{ind}, m_{val},} i, j)
  \\ [2pt]
  \angled{3, j}_{j \in [0, N)} : \mathtt{svi(x_{ind}, x_{val},} i)
  \end{array}
\!}
\hspec{\!\!\!
\left.
\begin{array}{r}
- \\[2pt] \many{m} \\[2pt] \many{x}
\end{array}
\right|
\begin{array}{l}
\exists a, \arr{ans(1)}{a} \str
\\[2pt]
\pure{\forall i, a[i] = \sum_j \many{m}(i,j)\many{x}(j)} 
\\[2pt]
\str \arrs \str \top  
\end{array}
\!\!\!}
}}
\end{equation}
%
The first line of the postcondition states that the result of the
computation stored in the array \code{ans} of the first component is a
dense vector~$a$ of the size $M$, while the second line asserts, in
the common mathematical notation, that $a$ is a result of multiplying
the dense representation of the matrix $\many{m}$ by the corresponding
dense vector~$\many{x}$.
%
We slightly abuse the hyper-value notation by referring to elements of
$\many{m}$ in the postcondition as $\many{m}(i, j)$, assuming the
natural lexicographic order on the elements of the corresponding index
set $\set{\angled{2, i, j}~|~ i \in [0, M), j \in [0,N)}$.

\subsection{Verifying Sparse Multiplication}
\label{sec:verify-sparse-mult}

The proof of \eqref{eq:csr1} is best explained in two steps, each
focusing on one of \code{spmspv}'s loops.

\subsubsection{Step 1: Top-Level \code{for}-Loop Decomposition}

The body of \code{spmspv} is represented by a loop that iterates
through all rows of the matrix~$m$ via the variable~\code{i}:
%
\begin{equation}
\label{eq:csr2}
{\small{
\hspec{\!\!\!
\begin{array}{c}
  \arr{ans(1)}{\Zero} 
  \\[2pt]
  \str~\arrs  
\end{array}
\!\!\!}    
\hmid{\!\!\!
  \begin{array}{c@{\ }c@{\ }l}
  1 : \forl{i}{0}{|\inds{m}|}{p(i)}
  \\ [2pt]
  \angled{2, i, j}_{\!\!\!\!\tiny
    \begin{array}{l} i \in [0, M) \\ j \in [0,N) \end{array}} :  \mathtt{csrij(m_{ind}, m_{val},} i, j)
  \\ [2pt]
  \angled{3, j}_{j \in [0, N)} : \mathtt{svi(x_{ind}, x_{val},} j) 
  \end{array}
\!}
\hspec{\!\!\!
\left.
\begin{array}{r}
- \\[2pt] \many{m} \\[2pt] \many{x}
\end{array}
\right|
\begin{array}{l}
\exists a, \arr{ans(1)}{a} \str
\\[2pt]
\pure{\forall i, a[i] = \sum_j \many{m}(i,j)\many{x}(j)} 
\\[2pt]
\str \arrs \str \top  
\end{array}
\!\!\!}
}}
\end{equation}
%
Each iteration of the \code{for}-loop handles exactly one row of $m$,
computing the value of multiplying it by all values of~$x$, encoded
via \code{x_ind} and \code{x_val}.
%
To proceed with our proof, we employ the general form of the
\rulename{For} rule, as depicted in~\autoref{log:loop}.
%
The simplified version of this rule from \autoref{fig:seq}, which we
used to verify a sum over an RL-compressed array in \autoref{sec:for},
allowed only for a \emph{disjoint} split of the format-related index
set to match individual iterations of the \code{for}-loop in the main
program.
%
In contrast, the general form of the rule from \autoref{log:loop}
allows for splitting the index set into possibly overlapping
components, assuming that the loop invariant only restricts the part
of the hyper-state ascribed to the main program component. Luckily,
this is exactly the case for this example, where we can define the
invariant $\Ifor(i, \many{m}\many{x})$ for the \code{for}-loop as
follows:
%
\begin{equation*}
{\small{
  \Ifor(i, \many{m}\many{x}) \eqdef  
  \bigstr_{k = 0}^{i - 1} \Ans(1) + k \mapsto \sum_j\many{m}(i,
  j)\many{x}(j) \str
  \bigstr_{k = i}^{M - 1} \Ans(1) + k \mapsto 0
}}
\end{equation*}
%
Notice that the invariant above only constraints the hyper-state
relevant to the component 1.
%
Next, we represent the index sets of the auxiliary format components
as the following two unions:
%
\vspace{-5pt}
%
{\small{
\begin{align*}
\set{
\angled{2, i, j}~\left|
\begin{array}{l} i \in [0, M) \\ j \in [0,N) \end{array}
\right.
} &= \biguplus_{i = 0}^{M - 1} \set{\angled{2, i, j}~|~j \in [0,N)}
\\
\set{\angled{3, j}~|~{j \in [0, N)}} &= 
\bigcup_{0}^{M - 1} \set{\angled{3, j} ~|~ {j \in [0, N)}}
\end{align*}
%
}}
%
%\vspace{-5pt}
%
\noindent
%
That is, while the first set has been split into $M$ disjoint
components, the second has been represented as a union of $M$ its own
identical copies, as we will need it for \emph{each} of $M$ iterations
of the \code{for}-loop.
%
Choosing the invariant $\Ifor$ and the split as above leads to the
following proof obligation, after framing out all the unchanged
components of the state in the invariant:
%
\begin{equation}
\label{eq:csr3}
{\small{
\hspec{\!
\begin{array}{c}
  \Ans(1)+i \mapsto 0
  \\[2pt]
  \str~\ldots  
\end{array}
\!}    
\hmid{\!\!\!
  \begin{array}{c@{\ }c@{\ }l}
  1 &:& p(i)
  \\ [2pt]
  \angled{2, i, j}_{j \in [0, N)} &:&  \mathtt{csrij(m_{ind}, m_{val},} i, j)
  \\ [2pt]
  \angled{3, j}_{j \in [0, N)} &:& \mathtt{svi(x_{ind}, x_{val},} j) 
  \end{array}
\!}
\hspec{\!
\left.
\begin{array}{r}
- \\[2pt] \many{m} \\[2pt] \many{x}
\end{array}
\right|
\begin{array}{c}
{\Ans(1) + i} \mapsto \sum_j \many{m}(i,j)\many{x}(j) 
\\[2pt] \str \ldots
\end{array}
\!}
}}
\end{equation}
%
In~\eqref{eq:csr3}, the implicitly universally quantified variable $i$
ranges from $0$ up to $|\inds{m}| - 1$.
%
Since $i$ is fixed across all the programs in the second component
product, let us re-index it, simultaneously rewriting the call to
\code{csrij} with its definition (also notice a subtle change in using
$\many{m}$ in the postcondition):
%
%
\begin{equation}
\label{eq:csr4}
{\small{
\hspec{\!
\begin{array}{c}
  \Ans(1)+i \mapsto 0
  \\[2pt]
  \str~\ldots  
\end{array}
\!}    
\hmid{\!\!\!
  \begin{array}{c@{\ }c@{\ }l}
  1 &:& p(i)
  \\ [2pt]
  \angled{2, j}_{j \in [0, N)} &:&  \mathtt{svi(m_{ind}[i], m_{val}[i],} j)
  \\ [2pt]
  \angled{3, j}_{j \in [0, N)} &:& \mathtt{svi(x_{ind}, x_{val},} j) 
  \end{array}
\!}
\hspec{\!
\left.
\begin{array}{r}
- \\[2pt] \many{m} \\[2pt] \many{x}
\end{array}
\right|
\begin{array}{c}
{\Ans(1) + i} \mapsto \sum_j \many{m}(j)\many{x}(j) 
\\[2pt] \str \ldots
\end{array}
\!}
}}
\end{equation}
%
Progressing beyond line~3 of \code{spmspv} and allocating the
variable \code{iM} and \code{iX} leaves with the goal:
%
\begin{equation}
\label{eq:csr5}
{\small{
\!\!\!\!
\hspec{\! \! 
  \begin{array}{c}
    {\tt ans(1)}+i \mapsto 0 \str\!\! \\[2pt]
    \mcode{iX} \mapsto 0 \str
    \mcode{iM} \mapsto 0 \str \\[2pt]
    \ldots 
  \end{array}
\!\! \!}    
\hmid{\!\!\!
  \begin{array}{c@{\ }c@{\ }l}
  1 &:& \kw{while}\ (\dots) \{\dots\}
  \\ [2pt]
  \angled{2, j}_{j \in [0, N)} &:&  \mathtt{svi(m_{ind}[i], m_{val}[i],} j)
  \\ [2pt]
  \angled{3, j}_{j \in [0, N)} &:& \mathtt{svi(x_{ind}, x_{val},} j) 
  \end{array}
\!}
\hspec{\! \! \!
\left.
\begin{array}{r}
- \\[2pt] \many{m} \\[2pt] \many{x}
\end{array}
\right|
\begin{array}{c}
{\Ans(1) + i} \mapsto \sum_j \many{m}(j)\many{x}(j) 
\\[2pt] \str \ldots
\end{array}
\! \!\!}
}}
\end{equation}
%
To proceed further, let us make an important observation.
%
Remember that both arrays $\inds{m}[i]$ and $\inds{x}$ contain indices
of non-zero elements of the corresponding dense vectors. 
%
Therefore any elements of those vectors positioned at indices larger
than $\St = \min(\max(\inds{m}[i]), \max(\inds{x}))$ will \emph{not}
contribute to the sum stored in \code{ans(1)} due to either being
zero or being multiplied by zero.
%
This fact can be phrased as the following hyper-safety triple:
%
\begin{equation}
\label{eq:csr6}
  {\small{
  \hsll
  { \!\! \dots \begin{array}{l}\phantom{a}\\[2pt]\phantom{a}\end{array} \!\! \!\! \!\! \!\! \!\! \!\!\! }
  {
  \!\!
  \begin{array}{c@{\ }c@{\ }l}
  \angled{2,j}_{\St < j < N} &:&  \mathtt{svi(m_{ind}[i], m_{val}[i],} j)
  \\ [2pt]
  \angled{3,j}_{\St < j < N} &:& \mathtt{svi(x_{ind}, x_{val},} j) 
  \end{array}
  \!\!
  }
  {\many{m} \\ \many{x}}
  {\!\!  \pure{\forall j > \St,\ \many{m}(j)\many{x}(j) = 0} \!\!}  
  }}
\end{equation}
%
Using the rule \rulename{SeqU} (\autoref{fig:seq}) we can, therefore,
reduce~\eqref{eq:csr5} to the following goal:
%
\begin{equation}
\label{eq:csr7}
{\small{
\!\!\!\!
\hspec{\! \! 
  \begin{array}{c}
    {\tt ans(1)}+i \mapsto 0 \str\!\! \\[2pt]
    \mcode{iX} \mapsto 0 \str
    \mcode{iM} \mapsto 0 \str \\[2pt]
    \ldots 
  \end{array}
\!\! \!}    
\hmid{\!\!\!
  \begin{array}{l}
  \phantom{a}~1 : \kw{while}\ \mcode{(cond(iM,iX))} \set{\ldots}
  \\ [2pt]
  \angled{2,j}_{j \leq \St} :  \mathtt{svi(m_{ind}[i], m_{val}[i],} j)
  \\ [2pt]
  \angled{3,j}_{j \leq \St} : \mathtt{svi(x_{ind}, x_{val},} j) 
  \end{array}
\!}
\hspec{\! \! \!
\left.
\begin{array}{r}
- \\[2pt] \many{m} \\[2pt] \many{x}
\end{array}
\right|
\begin{array}{c}
{\Ans(1) + i} \mapsto \sum_{j\leq st} \many{m}(j)\many{x}(j) 
\\[2pt] \str \ldots
\end{array}
\! \!\!}
}}
\end{equation}
%
where \code{cond(iM, iX)} abbreviates the actual condition of the
\code{while}-loop in line~4 of \autoref{fig:smpv}.

\subsubsection{Step 2: Verifying the \code{while}-loop}
%
We are going to use the general \rulename{While} rule to verify the
goal~\eqref{eq:csr7}.
%
Recall from \autoref{subsec:loops} that this rule in \logic provides
access to the \emph{counting} aspect of a \code{while}-loop.
%
This is thanks to the second parameter~$s$ of its invariant of the
shape $\Iwl(b, s, \many{v})$ that ``keeps track'' of the number of
(format-related) auxiliary program components aligned with the
previous loop iterations.
%
The first invariant parameter, $b$, keeps the status of the loop
condition, while the last, $\many{v}$ accumulates the hyper-value
containing the results of the auxiliary programs executed in alignment
with the past iterations.

To make use of the rule for our example, we choose the following invariant:
%
\begin{equation} 
\label{eq:csr8}
  \small{
  \begin{array}{r@{\ }c@{\ }l@{\ }l}
    \Iwl(b, s,\many{m}\many{x}) & \eqdef 
   & \exists \Imm, \Ixx, & \mcode{iM} \mapsto\Imm \str \mcode{iX}
                           \mapsto \Ixx \str \mcode{cond}(\Imm, \Ixx) \Leftrightarrow b \str \\[2pt]
   &&& \pure{\min(\inds{x}[\Ixx], \inds{m}[i][\Imm]) = s} \str\\[2pt]
   &&& \Ans(1) + i \mapsto \sum_{j < s} \many{m}(j)\many{x}(j) \str \dots \\[2pt]
  \end{array}}
\end{equation}
%
The first line of the invariant simply gives names to the values
stored in the vector counters ($\Imm$~and~$\Ixx$) and relates their
values to the loop condition $b$.
%
The second line is the most subtle:
%
it captures the overall ``progress'' through the pair of the dense
vectors being multiplied by storing the minimum of $\inds{x}[ix]$ and
$\inds{m}[i][im]$ in the variable $s$, which, according to the rule
premises, also counts the number of auxiliary programs ``dispatched''
by that time.
%
This assertion is crucial for recording the \emph{lower boundary} for
the index~$j$ determining which components to include for alignment
with the current loop iteration and what portion of the product of the
two vectors has been already accumulated in the location $\Ans(1) + i$
of the result (last assertion in \eqref{eq:csr8}).

Abbreviating the body of the \code{while}-loop as~$q$ and applying the
rule \rulename{While} gives us the following:
%
\begin{equation}
\label{eq:csr9}
  {\small{
  \hsll
  { \!\! 
  \Iwl(\True, s, \many{m}\many{x}) \!\!\! }
  {
  \!\!
  \begin{array}{c@{\ }c@{\ }l}
  1 &:& q; \kw{while}(\mcode{cond(iM, iX)})~\set{q}
  \\ [2pt]
  \angled{2,j}_{s \leq j \leq \St} &:&  \mathtt{svi(\inds{m}[i], \vals{m}[i],} j)
  \\ [2pt]
  \angled{3,j}_{s \leq j \leq \St} &:& \mathtt{svi(\inds{x}, \vals{x},} j) 
  \end{array}
  \!\!
  }
  {- \\ \many{m} \\ \many{x}}
  {\!\! 
  {\Iwl(\False, \St+1, \many{m}\many{x})\!\!}  
  }}}
\end{equation}
%
Since the body of the loop is an \code{if}-statement, the rest of the
proof proceeds by case analysis.

In the first case, $\xind[ix] = \mind[im]$. Let us define
$s' \eqdef \min(\xind[ix+1],\mind[im+1])$, which will be a new value
of the ``auxiliary program counter'' $s$ after this iteration.
%
This brings us to
%
\begin{equation}
\label{eq:csr10}
{\small{
    \hsll
    { \!\! 
      \Iwl(\True, s, \many{m}\many{x}) \!\!\! }
    {
      \!\!
      \begin{array}{c@{\ }c@{\ }l}
        1 &:& q
        \\ [2pt]
        \angled{2,j}_{j \in [s,s')} &:&  \mathtt{svi(\inds{m}[i], \vals{m}[i],} j)
        \\ [2pt]
        \angled{3,j}_{j \in [s,s')} &:& \mathtt{svi(\inds{x}, \vals{x},} j) 
      \end{array}
      \!\!
    }
    {- \\ \many{m}' \\ \many{x}'}
    {\!\! 
    {\Iwl(b', s', \many{m}'\many{m}\many{x}'\many{x})\!\!}  
    }}}
\end{equation}
%
The postcondition of~\eqref{eq:csr10} will therefore serve as a
precondition to the induction hypothesis about the next iteration of
the \code{while}-loop from the premise of the \rulename{While} rule.
%
Furthermore, the statement of~\eqref{eq:csr10} means that the current
iteration of the body of the loop will process all elements $x[i]$
and $m[i][j]$ in a pair-wise fashion for all~$j$ such that
$s \leq j < s'$.
%
Tho prove this goal, let us execute $q$ to completion, updating the
values of \code{ans}, \code{iM}, and \code{iX}, resulting in the
following goal, where $y$ binds the accumulated sum
$\sum_{j < s} \many{m}(j)\many{x}(j)$ and all irrelevant parts of the
invariant are omitted:
%
\begin{equation}
\label{eq:csr11}
{\small{
    \hsll
    { \!\! 
      \Ans(1) + i \mapsto
      \\[2pt] 
      \phantom{aaaa} y + \xind[\Ixx]\mind[\Imm]
      \\[2pt] 
      \str \ldots \!\!\! }
    {
    \!\!
    \begin{array}{c}
    1 : \mcode{skip}  
    \\ [2pt]
    \angled{2,j}_{j \in [s,s')} :  \mathtt{svi(\dots})
    \\ [2pt]
    \angled{3,j}_{j \in [s,s')} : \mathtt{svi(\dots}) 
    \end{array}
    \!\!
    }
    {- \\ \many{m}' \\ \many{x}'}
    {\!\! 
    \begin{array}{l}
      \Ans(1) + i \mapsto 
      \\[2pt]
      \phantom{aaaa} y + \sum_{j = s}^{s'-1} \many{m}'(j)\many{x}'(j) 
      \\[2pt]
       \str \ldots
    \end{array}
    
    }}}
\end{equation}
%
We prove this goal by showing that $\xval[\Ixx]$ and $\mval[\Imm]$ are
the only \emph{simultaneously} non-zero values of~$\many{x}'$
and~$\many{m'}$.
%
Recall that $s = \xind[\Ixx] = \mind[\Imm]$ and
$s' = \min(\xind[\Ixx+1], \mind[\Imm+1])$, which excludes both
$\xind[\Ixx+1]$ and $\mind[\Imm+1]$ from the domains of $\many{x}'$
and $\many{m'}$.

This fact can be derived from the following two complementary
specifications of \code{svi}:
%
\begin{equation}
\label{eq:svi1}
{\small{
    \hsll
    { \!\!\!
      \arrl{\mcode{ind}}{\ind}\str 
      \arrl{\mcode{val}}{\val} \str
        \pure{j = \ind[i]}
    \!\!\! }
    {
    \!\!
    \begin{array}{c@{\ }c@{\ }l}
    e :  \mcode{svi}(\mcode{ind}, \mcode{val}, j)
    \end{array}
    \!\!
    }
    {x}
    {\!\! 
      \pure{x = \val[i]}\str \ldots
    \!
    }}}
  \end{equation}
  \noindent
  \begin{equation}
    \label{eq:svi2}
    {\small{
    \hsll
    { \!\! 
      \arrl{\mcode{ind}}{\ind}\str 
      \arrl{\mcode{val}}{\val} \str
      \pure{j \notin \ind}
    \!\!\! }
    {
    \!\!
    \begin{array}{c@{\ }c@{\ }l}
    e :  \mcode{svi}(\mcode{ind}, \mcode{val}, j)
    \end{array}
    \!\!
    }
    {x}
    {\!\! 
    \begin{array}{l}
      \pure{x = 0}\str \ldots 
    \end{array}
    }}}
\end{equation}
%
The second specification can be used for any $j$, such that
$s < j < s'$, which implies that such $j$ is neither in $\xind$ nor in
$\mind$.
%
Both~\eqref{eq:svi1} and~\eqref{eq:svi2} can be derived in unary
separation logic.

%%%%%%%%%%%%%%%%%

In the second case for~\eqref{eq:csr9}, $\xind[\Ixx] < \mind[\Imm]$,
which makes the goal~\eqref{eq:csr10} true for
$s' = \min(\xind[\Ixx+1],\mind[\Imm])$. 
%
This is because there would be no non-zero values of
$\many{m}'(j)\many{x}'(j)$ for $j \in [s, s')$ as could be proven,
again, via \eqref{eq:svi1} and~\eqref{eq:svi2}.
%
The third case is analogous to the second one.

\subsection{Summary}

The proof of the specification~\eqref{eq:csr1} of \code{spmspv}
has exercised almost all rules of \logic, including a general version
of \rulename{For} for the top-level \code{for}-loop and a novel
\rulename{While} rule for its nested \code{while}-loop, in addition to
its capabilities as a Separation Logic, required to specify the
properties of the \code{svi} format description.
%
We did not fully mechanise this proof by the time of POPL'24
submission deadline, so we provide some of its omitted low-level
derivations in the supplementary appendix.





==> caseproof.tex <==
First note that if at least one of $x_{ind}$ or $m_{ind}[i]$ is empty, then $st$ would be the minium of maximums of empty array. Which id by our convention is -1. Hence two of index sets $\angled{2,j}_{j \leq st}$ and $\angled{3,j}_{j \leq st}$ are empty, and the while loop will never be executed. So the triple holds trivially.

Thus we assume that both of $x_{ind}$ and $m_{ind}[i]$ are not empty. Our full invariant is

\begin{equation*} {
  \small{
    I(b, s,\many{m},\many{x}) \eqdef 
\exists im\, ix,\ 
  \begin{array}{l}
  iM \mapsto im \str iX\mapsto ix \str \\[2pt]
  \pure{{\tt min}(x_0, m_0) = s} \str\\[2pt]
  {\tt ans} + i \mapsto \sum_{j < s} \many{m}(i,j)\many{x}(j) \str \\[2pt]
  {\tt cond}(im,ix) \leftrightarrow b \str \\[2pt]
  \pure{x_0 < m_0 \Rightarrow \forall m \in m_{ind}[i],\ m < m_0 \Rightarrow m < x_0} \\[2pt]
  \pure{m_0 < x_0 \Rightarrow \forall x \in x_{ind},\ x < x_0 \Rightarrow x < m_0}
  \end{array}}}
\end{equation*}

Where by $x_0$ and $m_0$ we denote $x_{ind}[ix]$ and $m_{ind}[i][im]$. Note that in our convention, for non-empty $s$, if $i \geq |s|$, $s[i]$ is define as the last value of $s$ plus one.

Last two conjuncts denote that $x_0$ and $m_0$ are in some sense closest values of $x_{ind}$ and $m_{ind}[i]$. For instance if $x_0 < m_0$, then $m_0$ is the smallest value of $m_{ind}[i]$ which is still greater that $x_0$.

We use the following division of our index set 

\[\small \angled{2,j}_{j \leq st} \cup \angled{3,j}_{j \leq st} = \biguplus_{j = 0}^{st} \{ \angled{2,j}, \angled{3,j} \} \]

Note that $I({\tt false}, s, \many{m},\many{x})$ implies that condition is false. Hence at least of one $im$ or $ix$ would be out of its bounds. Because of our convention one of $x_0$ or $m_0$ would be maximal element of the correspondent array plus one. Hence $s = st + 1$, and the post condition holds. 

Now, denoting the loop body with $p$, we have to show 

\begin{equation}
  \label{eq:goal}
  % \label{eq:rlprod2}
  {\small{
  \hsll
  { \!\! 
  I({\tt true}, s, \many{m},\many{x}) \!\!\! }
  {
  \!\!
  \begin{array}{c@{\ }c@{\ }l}
  1 &:& p
  \\ [2pt]
  \angled{2,j}_{j \geq s} &:&  \mathtt{svi(m_{ind}[i], m_{val}[i],} j)
  \\ [2pt]
  \angled{3,j}_{j \geq s} &:& \mathtt{svi(x_{ind}, x_{val},} j) 
  \end{array}
  \!\!
  }
  {\_ \\ \many{m} \\ \many{x}}
  {\!\! 
  {I(st, {\tt false}, \many{m}, \many{x})\!\!}  
  }}}
\end{equation}

Using 

\begin{equation}
  \label{eq:ih}
  % \label{eq:rlprod2}
  {\small{
  \hsll
  { \!\! 
  I({\tt true}, s', \many{m},\many{x}) \!\!\! }
  {
  \!\!
  \begin{array}{c@{\ }c@{\ }l}
  1 &:& p; w
  \\ [2pt]
  \angled{2,j}_{j \geq s'} &:&  \mathtt{svi(m_{ind}[i], m_{val}[i],} j)
  \\ [2pt]
  \angled{3,j}_{j \geq s'} &:& \mathtt{svi(x_{ind}, x_{val},} j) 
  \end{array}
  \!\!
  }
  {\_ \\ \many{m} \\ \many{x}}
  {\!\! 
  {I(st, {\tt false}, \many{m}, \many{x})\!\!}  
  }}}
\end{equation}

For some $s'$ greater then $s$.

Let $im$ and $ix$ be two current values of $iM$ and $iX$. We consider 2 cases: $x_{ind}[ix] = m_{ind}[im]$ and $x_{ind}[ix] > m_{ind}[iM]$. Third case when $x_{ind}[ix] < m_{ind}[im]$ is analogous to the second one.

\begin{enumerate}
  \item Let $x_{ind}[ix] = m_{ind}[im]$. Denote $s'$ to be ${\tt min}(x_{ind}[ix+1], m_{ind}[im+1])$. We show 
  \begin{equation}
    \label{eq:step1}
    {\small{
    \hsll
    { \!\! 
    I({\tt true}, s, \many{m},\many{x}) \!\!\! }
    {
    \!\!
    \begin{array}{c@{\ }c@{\ }l}
    1 &:& p
    \\ [2pt]
    \angled{2,j}_{j \in [s,s')} &:&  \mathtt{svi(m_{ind}[i], m_{val}[i],} j)
    \\ [2pt]
    \angled{3,j}_{j \in [s,s')} &:& \mathtt{svi(x_{ind}, x_{val},} j) 
    \end{array}
    \!\!
    }
    {\_ \\ \many{m_1} \\ \many{x_1}}
    {\!\! 
    {I(b', s', \many{m_1m}, \many{x_1x})\!\!}  
    }}}
  \end{equation}
  After we execute the loop body our pre-condition will become 
  \[\small 
    \begin{array}{l} 
       iM \mapsto im+1 \str iX \mapsto ix+1 \str \\[2pt]
       {\tt ans}+i \mapsto \dots + x_{val}[ix]m_{val}[im] 
    \end{array}\]
  We have to show that $\sum_{j \in [s,s')} \many{m_1}(i,j)\many{x}(j)$ equals to $x_{val}[ix]m_{val}[im]$, where $\many{m_1}$ and $\many{x_1}$ are results of correspondent $\tt svi$s. Which is trivial because the only values of $x_{ind}$ and $m_{ind}[i]$ in the interval $[s, s')$ are  $x_{ind}[ix]$ and $m_{ind}[im]$. 

  Now are left to show 
  \begin{equation*}
    % \label{eq:step1}
    \small{
     \begin{array}{l}
    \pure{x_0 < m_0 \Rightarrow \forall m \in m_{ind}[i],\ m < m_0 \Rightarrow m < x_0} \\[2pt]
    \pure{m_0 < x_0 \Rightarrow \forall x \in x_{ind},\ x < x_0 \Rightarrow x < m_0}
    \end{array}}
  \end{equation*}
  Where by $x_0$ and $m_0$ we denote $x_{ind}[ix+1]$ and $m_{ind}[i][im+1]$. This two facts are symmetric so we consider only the case when $x_0 < m_0$.
  Assume $m < m_0$. Then, because of the sortedness of $m_{ind}[i]$, we conclude $m \leq m_{ind}[i][im]$. We reach the conclusion by noticing:
  \[ m \leq m_{ind}[i][im] = x_{ind}[ix] < x_0\]
  \item Let $x_{ind}[ix] > m_{ind}[im]$. Because of the invariant we conclude 
  \begin{equation*} 
    \label{eq:aux}
    \forall x \in x_{ind}, x \geq x_{ind}[ix] \lor x < m_{ind}[i][im] 
  \end{equation*}
   Denote $s'$ to be ${\tt min}(x_{ind}[ix], m_{ind}[im+1])$. We show 
  \begin{equation}
    \label{eq:step2}
    {\small{
    \hsll
    { \!\! 
    I({\tt true}, s, \many{m},\many{x}) \!\!\! }
    {
    \!\!
    \begin{array}{c@{\ }c@{\ }l}
    1 &:& p
    \\ [2pt]
    \angled{2,j}_{j \in [s,s')} &:&  \mathtt{svi(m_{ind}[i], m_{val}[i],} j)
    \\ [2pt]
    \angled{3,j}_{j \in [s,s')} &:& \mathtt{svi(x_{ind}, x_{val},} j) 
    \end{array}
    \!\!
    }
    {\_ \\ \many{m_1} \\ \many{x_1}}
    {\!\! 
    {I(b', s', \many{m_1m}, \many{x_1x})\!\!}  
    }}}
  \end{equation}
  After we execute the loop body our pre-condition will become 
  \[\small 
    \begin{array}{l} 
       iM \mapsto im+1 \str iX \mapsto ix \str \\[2pt]
       {\tt ans}+i \mapsto \sum_{j < s} \dots
    \end{array}\]
  We have to show that $\sum_{j \in [s,s')} \many{m_1}(i,j)\many{x}(j)$ equals to 0, where $\many{m_1}$ and $\many{x_1}$ are results of correspondent $\tt svi$s. The only value of $m_{ind}[i]$ in $[s,s')$ is $m_{ind}[i][im]$. So 
  \noindent
  \[\sum_{j \in [s,s')} \many{m_1}(i,j)\many{x}(j) = \many{m_1}(i,m_{ind}[i][im]) \many{x_1}(m_{ind}[i][im]) \]
  \noindent
  However $m_{ind}[i][im]$ doesn't satisfy any disjuncts in~\eqref{eq:aux}. Hence $m_{ind}[i][im] \notin x_{ind}$. Hence $\many{x_1}(m_{ind}[i][im]) = 0$. And the summation is indeed 0.

  Now are left to show 
  \begin{equation*}
    \small{
     \begin{array}{l}
    \pure{x_0 < m_0 \Rightarrow \forall m \in m_{ind}[i],\ m < m_0 \Rightarrow m < x_0} \\[2pt]
    \pure{m_0 < x_0 \Rightarrow \forall x \in x_{ind},\ x < x_0 \Rightarrow x < m_0}
    \end{array}}
  \end{equation*}
  Where by $x_0$ and $m_0$ we denote $x_{ind}[ix]$ and $m_{ind}[i][im+1]$. Consider both cases
  \begin{enumerate}
    \item Let $x_{ind}[ix] < m_{ind}[i][im+1]$, and $m <  m_{ind}[i][im+1]$. Because of the sortedness of $m_{ind}[i]$, we have $m \leq m_{ind}[i][im]$. We reach the conclusion by noticing:
    \[ m \leq m_{ind}[i][im] < x_{ind}[ix] < x_0\]
    \item  Let $m_{ind}[i][im+1] < x_{ind}[ix]$ and $x <  x_{ind}[ix]$. Because of the invariant we conclude $x < m_{ind}[i][im]$. So as $m_{ind}[i]$ is sorted, $x < m_{ind}[i][im+1]$
  \end{enumerate}
\end{enumerate}
\noindent
Finally, combining~\eqref{eq:step1} in the first case and~\eqref{eq:step2} with~\eqref{eq:ih} we obtain~\eqref{eq:goal}.


==> discussion.tex <==

\section{Discussion}
\label{sec:discussion}

\is{Moved this part from the Overview. Please, elaborate}.


% TODO: Move to related works
% In LHC there is a rule that is used in such cases is \tname{wp-conj}. In~\cite{DOsualdoFD22} it is written as it depicted on~\autoref{img:wp-conj}.

% \begin{figure}
%   \begin{prooftree}
%     \AXC{idx\((Q_1) \subseteq \text{supp}(t_1)\)}
%     \AXC{idx\((Q_2) \subseteq \text{supp}(t_2)\)}
%     \RightLabel{\small \tname{wp-conj}}
%     \BIC{\( wp\ t_1\ \{ Q_1 \}\ \land\ wp\ t_2\ \{ Q_2 \}\ \vdash wp\ (t_1+t_2)\ \{Q_1 \land Q_2 \} \)}
%   \end{prooftree}
%   \caption{\tname{wp-conj} rule from~\cite{DOsualdoFD22}}
%   \label{img:wp-conj}
% \end{figure}

% Let's reformulate this rule in a separation-triple \logic style, and show the possible use case.

% \begin{prooftree}
%   \AXC{\small\(\hsll{P_1}{R:\ p}{\many{x}}{Q_1(\many{x}) }\)}
%   \AXC{\small\(\hsll{P_2}{S:\ p}{\many{x}}{ Q_2(\many{x}) }\)}
%   \RightLabel{\tname{\logic-conj}}
%   \BIC{\small\(\hsll{P_1 \land P_2}{R \cup S:\ p}{\many{x}}{Q_1(\many{x}) \land Q_2(\many{x}) }\)}
% \end{prooftree}

% If we decided to merge~\eqref{eq:rlf4} and~~\eqref{eq:rlf2} via \tname{\logic-conj}, we would have to prove the following post-condition entailment forall $\many{x} \in \Vec_{\angled{2, i}_{i \in [0, N)}}$:

% \[
%   \begin{array}{c}
%     s \mapsto \sum_i \many{x}(i) \str \top \\[2pt] \land \\[2pt]
%     \exists a, 
%         \begin{array}{l} 
%           s \mapsto \sum_i a[i]\ \str \\[2pt]
%           \arrl{x}{a} \str  \\[2pt]
%           \pure{\sum_i a[i] = \sum_i \many{x}(i)} \str \\[2pt] \top
%         \end{array}
%   \end{array} \Longrightarrow\ \ \  \exists a, 
%   \begin{array}{l} 
%     s \mapsto sum_i a[i]\ \str \\[2pt]
%     \arrl{x}{a} \str  \\[2pt]
%     \pure{\sum_i a[i] = \sum_i \many{x}(i)} \str \\[2pt] \top
%   \end{array}
%   \]

% Which is valid, but requires reasoning about conjunction in Separation logic \vg{BAD!}.

% So, if we want to avoid conjunction, we have to come up the alternative for \tname{\logic-conj}. 



==> figtriples.tex <==
\begin{equation*}
  % \label{eq:spmspv2}
  {\small{
  \hspec{\!\!\!
  \begin{array}{c}
    \bigstr_{i=0}^M \code{ans(1)}+i\mapsto 0
    \\
    \str \arrs(\cdot)
  \end{array}
  \!\!\!}    
  \hmid{\!\!\!
    \begin{array}{c@{\ }c@{\ }l}
    1 &:& \forl{i}{0}{|\idxs{m}|}{p(i)}
    \\ [2pt]
    \angled{2, i, j}_{\!\!\!\!\tiny
    \begin{array}{l} i \in [0, M) \\ j \in [0,N) \end{array}} &:&  \mathtt{ucsr\_get(m_{idx}, m_{ind}, m_{val},} i, j)
    \\ [2pt]
    \angled{3, j}_{j \in [0,N)} &:& \mathtt{sv\_get(x_{ind}, x_{val},} j)
    \end{array}
  \!}
  \hspec{\!\!\!
  \left.
  \begin{array}{r}
  - \\[2pt] \many{m} \\[2pt] \many{x}
  \end{array}
  \right|
  \begin{array}{l}
  \exists s, \bigstr_{i=0}^M \code{ans(1)}+i\mapsto s[i] \str
  \\[2pt]
  \pure{\forall i, s[i] = \sum_j \many{m}(i,j)\many{x}(j)} 
  \\[2pt]
  \str \arrs(\cdot) 
  \end{array}
  \!\!\!}
  }}
\end{equation*}

\begin{equation*}
  \label{eq:spmspv3}
  {\small{
  \hspec{\!\!\!
  \begin{array}{c}
    \bigstr\limits_i \code{ans(1)}+i\mapsto 0 \\[-2pt]
    \str \arrs(\cdot)
  \end{array}
  \!\!\!}    
  \hmid{\!\!\!
    \begin{array}{c@{\ }c@{\ }l}
    1 &:& \forl{i}{0}{|\idxs{m}|}{p(i)}
    \\ [2pt]
    \angled{2, i, j}_{\!\!\!\!\tiny
    \begin{array}{l} i \in \idxs{m} \\ j \in [0,N) \end{array}} &:&  \mathtt{ucsr\_get(m_{idx}, m_{ind}, m_{val},} i, j)
    \\ [2pt]
    \angled{3, j}_{j \in [0,N)} &:& \mathtt{sv\_get(x_{ind}, x_{val},} j)
    \end{array}
  \!}
  \hspec{\!\!\!
  \left.
  \begin{array}{r}
  - \\[2pt] \many{m} \\[2pt] \many{x}
  \end{array}
  \right|
  \begin{array}{l}
  \bigstr\limits_{i \in \idxs{m}}\!\!\code{ans(1)}+i\mapsto \\[-6pt]
  \qquad\quad \sum_j \many{m}(i,j)\many{x}(j)
  \\[2pt]
  \bigstr\limits_{i \not\in \idxs{m}}\!\!\code{ans(1)}+i\mapsto 0
  \\[2pt]
  \str \arrs(\cdot) 
  \end{array}
  \!\!}
  }}
\end{equation*}

\begin{equation}
  \label{eq:spmspv4}
  {\small{
  \hspec{\!\!\!
  \begin{array}{c}
    \arrs(\cdot)
  \end{array}
  \!\!\!}    
  \hmid{\!\!\!
    \begin{array}{c@{\ }c@{\ }l}
    \angled{2, i, j}_{\!\!\!\!\tiny
    \begin{array}{l} i \not\in \idxs{m} \\ j \in [0,N) \end{array}} &:&  \mathtt{ucsr\_get(\dots} i, j)
    \end{array}
  \!}
  \hspec{\!\!\!
  \begin{array}{r}
  ~~\many{m}
  \end{array}
  \!\!\left|
  \begin{array}{l}
  \pure{\forall i \notin \idxs{m}\, \forall j, \many{m}(i,j) = 0}
  \\[2pt]
  \str \arrs(\cdot) 
  \end{array}
  \right.
  \!\!\!}
  }}
\end{equation}

==> figures/altogether.tex <==
\scalebox{0.77}{
\begin{minipage}{1.0\linewidth}
{\small{
\!\!\!\! \!\!\!\! \!\!\!\! \!\!\!\!
\begin{mathpar}
\inferrule* [Right=$\begin{array}{c}
\!\!\!\!\text{\rulename{Merge}, \rulename{Proj} ({\S}\ref{sec:merge})}
\arcr 
\!\!\!\!\text{\rulename{Sep} ({\S}\ref{sec:switch})} 
\end{array}$]
{
  \inferrule* [Left={\rulename{SeqU1}~({\S}\ref{sec:seq})}]
  {
  \inferrule* [Left={\rulename{For}~({\S}\ref{sec:for})}]
    {
      \inferrule* [Left={\rulename{SeqU}~({\S}\ref{sec:for})}]
      {
        \inferrule*[Left={SepLog~({\S}\ref{sec:unary})}]
        {\inferrule{\ldots}{\kw{while}\ (\tinds{x}[j+1] \leq k)\ \set{j\text{++}}}}
        {\angled{3, k} : \mathtt{rli}(\tinds{x}, \tvals{x}, k)    }   
      }
      {
       \hmid{\!\!\!
       \begin{array}{c}
         2 :  \kw{if} (k+1 \geq \tinds{x}[a+1])\ \set{\ldots}
        \\ [2pt]
        \angled{3, k}_{k \in \ldots} : \mathtt{rli}(\tinds{x}, \tvals{x}, k)    
        \end{array}\!\!\!}    
      }
     }
   {
   \hmid{\!\!\!
   \begin{array}{c}
    2 : \forl{k}{0}{N}{\dots}
    \\ [2pt]
    \angled{3, j}_{j \in \ldots} : \mathtt{rli}(\tinds{x}, \tvals{x}, j)    
   \end{array}\!\!\!}    
   }
  }
  {
   \hmid{\!\!\!
   \begin{array}{c}
    2 :  \mathtt{rl}(\tinds{x}, \tvals{x}, N)
    \\ [2pt]
    \angled{3, j}_{j \in \ldots} : \mathtt{rli}(\tinds{x}, \tvals{x}, j)    
   \end{array}\!\!\!}    
  }
\quad
  \inferrule*[Right={
    \begin{tabular}{l}
    \rulename{SeqU1}\\ \rulename{SeqU2}  
    \end{tabular}({\S}\ref{sec:rlispec})}]
  {\inferrule*[Right={\rulename{For}~({\S}\ref{sec:rlispec})}]
   {
     \inferrule*[Right={\rulename{SeqU}~({\S}\ref{sec:rlispec})}]
     { 
       \inferrule{\ldots}{\mathtt{s}~{\text{+=}}~\tvals{x}[i] * (\ldots) }
       \\
       \inferrule*[Right={\rulename{Prod}~({\S}\ref{sec:independent})}]
       {
         \inferrule*[Right={SepLog~({\S}\ref{sec:unary})}]
         {
           \inferrule{\ldots}{\kw{while}\ (\tinds{x}[j+1] \leq k)\ \set{j\text{++}}}
         }
         {\hmid{\angled{2, k}} : \mathtt{rli}(\tinds{x}, \tvals{x}, k)}
       }
       {\hmid{\angled{2, j}}_{j \in \ldots} : \mathtt{rli}(\tinds{x}, \tvals{x}, j)}
     }
     {
       \hmid{\!\!\!
         \begin{array}{c}
           1 : \mathtt{s}~{\text{+=}}~\tvals{x}[i] * (\ldots) 
           \arcr [2pt]
           \angled{2, j}_{j \in \ldots} : \mathtt{rli}(\tinds{x}, \tvals{x}, j)    
         \end{array}\!\!\!}
     }
   } 
   {\hmid{\!\!\!
   \begin{array}{c}
    1 : \forl{i}{0}{|\tinds{x}|}{\dots}
    \arcr [2pt]
    \angled{2, j}_{j \in \ldots} : \mathtt{rli}(\tinds{x}, \tvals{x}, j)    
   \end{array}\!\!\!}}
  }
  {
  \hmid{\!\!\!
   \begin{array}{c}
    1 : \mathtt{rlsum}(\tinds{x}, \tvals{x}) 
    \\ [2pt]
    \angled{2, j}_{j \in \ldots} : \mathtt{rli}(\tinds{x}, \tvals{x}, j)    
   \end{array}\!\!\!}
  }
}
{
\hmid{
\!\!
\begin{array}{l@{\ }c@{\ }l}
1 &: & {\mathtt{rlsum}}(\tinds{x}, \tvals{x}) 
\\ [2pt]
2 &: & {\mathtt{rl}}(\tinds{x}, \tvals{x}, N)    
\end{array}
\!\!
}
}
\end{mathpar}
}}
\end{minipage}
}



==> figures/for-rule.tex <==
\begin{figure}[t]
% \setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{-5pt}
{  \small{
   \begin{subfigure}{\textwidth}
    % \vspace{2mm}
    \begin{prooftree}
      \AXC{\(\forall j < N, \forall \many{x},\ \local{I(j,\many{x})}{\iota}\)}
      \AXC{\(S = \bigcup_{i=0}^{N - 1} S_i \)}
      \AXC{ \(\forall i < N,\ \local{R_i}{S_i}\)}
      \noLine
      \TIC{\(\forall \many{x}, i < N,
            \hsllazy{
              I(i, \many{x}) \str
              R_i \ \ }
              {\iota : p,~~S_i : \pp_i}
              {z, \many{y}}
              {I(i+1, \many{x}\many{y})
               \str \top_{S_i} }\)}
      \RightLabel{\rulename{For}}
      \UIC{\(\hsllazy{
                I(0, \many{\emptyset}) \str
                \bigstr_{i=0}^{N - 1} R_i \ \ }
                {\iota : \forl{i}{0}{N}{p},\
                 S : \pp}
                {z, \many{y}}
                {I(N, \many{y})
                 \str \top } \)}
    \end{prooftree}
  \end{subfigure}
}}
\caption{Rule for \code{for}-loops}
\label{log:loop}
\end{figure}


==> figures/while-rule.tex <==
\begin{figure}[t]
% \setlength{\abovecaptionskip}{5pt}
% \setlength{\belowcaptionskip}{-5pt}
{\small{
\!\! \!\!
  \begin{subfigure}{\textwidth}
    \vspace{4mm}
    \begin{prooftree}
      \AXC{\(\forall n,\ S_n \eqdef \biguplus_{i=n}^M S'_i\)}
      \noLine
      \UIC{\(\forall m\, \many{x},\ I(\False, m, \many{x}) \Rightarrow \pure{m = M}\!\str\!Q(\many{x})\)}
      \noLine
      \UIC{\(
        \begin{array}{l}
          \vspace{-13mm}
          \forall b\, m\, \many{x},\
          \hslc
          {I(b, m,\many{x})}
          {\iota:\, c}{b'}{
          \begin{array}{l} 
            I(b,m,\many{x})\!\\[2pt]\!\str\!\pure{b'=b}\!
          \end{array}
          }
          \end{array}
          \)}
      \AXC{\(
      \begin{array}{c}
        \forall m\, \many{x},~~
        \left(
          \begin{array}{l}
            \forall n \in (m,M]\ b\ \many{y}, \\[2pt]
            \hslcc{I(b,n,\many{y})}
            {\!\!\!\begin{array}{l} \iota\ \ \, : w \\ S_n:\pp \end{array}\!\!\!}
            {Q} 
          \end{array} \right)\Rightarrow \\[2pt]
        \hslcc
        {I(\True, m,\many{x})}
        {\!\!\!\begin{array}{l} 
          \iota:\ p;\ w \\[2pt]
          S_m: \pp
        \end{array}\!\!\!}{Q}
      \end{array}\)}
      \RightLabel{\rulename{While}}
      \BIC{\(\hslcc{\ I(\True, 0, \many{\emptyset})\ }{\iota:\kw{while}(c)\{p\},\ \bigcup_{i=0}^M S'_i :\pp }{Q}\)}
    \end{prooftree}
  \end{subfigure}
}}
\caption{A rule for \code{while}-loops}
\label{log:while}
\end{figure}


==> for-general.tex <==
\paragraph{General For-loop rule}


In order to understand why \tname{ForDisj} might not work in general we consider a different program.

Assume we have two functions $\tt f(i)$ and $\tt g(i)$, both returning an integer.

We want to prove that the following holds

\begin{equation*}
  % \label{eq:sumprod}
  \hsllazy
  {\!x(1)\mapsto 0\ \ }
  {1&:& \forl{i}{0}{n}{x\ {\text{\fontsize{9}{18}\selectfont +=}}\ {\tt f}(0) * {\tt g}(1)} \\[2pt]
   2&:& f(0) \\[2pt]
   3&:& g(1)}
  {\_ \\ v \\ u}
  {x(1)\mapsto n\cdot v \cdot u \! }
\end{equation*}

It would be nice if we could rewrite our goal like 

\begin{equation*}
  % \label{eq:sumprodS}
  \hsllazy
  {\!x(1)\mapsto 0\ \ }
  {1&:& \forl{i}{0}{n}{x\ {\text{\fontsize{9}{18}\selectfont +=}}\ {\tt f}(0) * {\tt g}(1)} \\[2pt]
   2&:& f(0) \\[2pt]
   3&:& g(1)}
  {\_ \\ v \\ u}
  {x(1)\mapsto \sum_{i=0}^n v \cdot u \! }
\end{equation*}

and apply \tname{ForDisj} here and reduce the goal to something like

\begin{equation*}
  % \label{eq:sumprod}
  \hsllazy
  {\!x(1)\mapsto y\ \ }
  {1&:& {x\ {\text{\fontsize{9}{18}\selectfont +=}}\ {\tt f}(0) * {\tt g}(1)} \\[2pt]
   2&:& f(0) \\[2pt]
   3&:& g(1)}
  {\_ \\ v \\ u}
  {x(1)\mapsto y + v \cdot u \! }
\end{equation*}

But remember, in order to do that, we have to partition the set of programmes (in this case $\{2\}$ and $\{3\}$) into $n$ \emph{disjoint} sets, and only then group each of those partition sets with each iteration of the for-loop. The sort of partition we want in this case is 
\begin{align*}
  \{2\} =& \bigcup_{i = 0}^n \{2\} \\
  \{3\} =& \bigcup_{i = 0}^n \{3\}
\end{align*}

Which is not disjoint.

So the trick we apply to overcome this issue is: we fist copy our programs $\tt f$ and $\tt g$ $n$-times, and change our post-condition to use results of each such copy:
\begin{equation*}
  % \label{eq:sumprodS}
  \hsllazy
  {\!x(1)\mapsto 0\ \ }
  {1: \forl{i}{0}{n}{x\ {\text{\fontsize{9}{18}\selectfont +=}}\ {\tt f}(0) * {\tt g}(1)} \\[2pt]
   \angled{2,i}_{i \in[0,n)}: f(0) \\[2pt]
   \angled{3,i}_{i \in[0,n)}: g(1)}
  {\_ \\ \many{v} \\ \many{u}}
  {x(1)\mapsto \sum_{i=0}^n \many{v}(i) \cdot \many{u}(i) \! }
\end{equation*}

This step can be justified by applying \tname{Merge} rule with 

\[\pi : \{1\} \cup \{2,3\}\times[0,n] \to \{1,2,3\} :=\] 
\[\lambda\ x,\
\begin{cases}
  1, & x = 1 \\
  2, & x = \angled{2, i} \text{ for some } i \\
  3, & x = \angled{3, i} \text{ for some } i 
\end{cases}\]

And then applying the \tname{ForDisj} rule assuming

\begin{align}
  \small
  R_i :=& emp \\
  S_i :=& \{\angled{2,i}, \angled{3,i}\} \\
  I(j,\many{y}) :=& x(1) \mapsto \sum_{i=0}^j \many{y}(i)
\end{align}

Actually the whole trick can be incorporated in the $\tt for$ rule, relaxing the condition on partition disjointedness, yielding a new rule~\hyperlink{rule:for}{\tname{For}}:

\vspace{-5mm}

\begin{figure}[h]
  \caption*{{\small\tname{For}} \phantom{kkkkkkkkkkkkkkkkkkkkkkkkkkkkkkkkkkkkkkkkkkkkkkkk}}
\begin{prooftree}
  % \AXC{\footnotesize $\forall j < N\ \forall \many{x},\ \local{I(j,\many{x})}{j}$}
  % \noLine
  \AXC{\small \(\forall j < N\ \forall \many{y},\ \local{I(j,\many{y})}{i}\)}
  \noLine
  \UIC{\small $S = \bigcup_{i=0}^N S_i$}
  \AXC{\small \(\forall j < N,\ \local{R_j}{S_i}\)}
  \noLine
  \UIC{ \small 
  \(%\begin{array}{l}
    \forall j < N\ \forall \many{x},\ %\in \Vec_{\biguplus_{i=0}^j S_i}, \vspace{3mm} \\[2pt]
    \hsllazy{
      I(j, \many{x}) \str
      R_j \ \ }
      {i &:& p \\[2pt]
       S_j &:& \pp}
      {\_ \\ \many{y}}
      {I(j+1, \many{x}\many{y})
       \str \top_{S_j} }
  %\end{array}
  \) }
  \BIC{
    \small
    \(\hsllazy{
      I(0, \mathbf{0}) \str 
      \bigstr_{i=0}^N R_i \ \ }
      {i :\ \forl{j}{0}{N}{p},\
       S :\ \pp}
      {\_\ \  \many{y}}
      {I(N, \many{y})
       \str \top }
      \)
  }
  \hypertarget{rule:for}{}
\end{prooftree}
\end{figure}



==> intro-old.tex <==
%\begin{itemize}
  % \item Structured data has become ubiquitous and is pervasive across various domains such as machine learning, routing, and many others. Efficiently representing structured or sparse data often involves identifying patterns of repetition, symmetry, or redundancy within the data. By leveraging these observations, the data can be compressed, removing unnecessary redundancy while introducing metadata that facilitates the reconstruction of the original data. Different ways of facilitating different patterns are called structured data ``formats''. Metadata, introduced my this formats be denoted as ``format components''.
  % \item Computing on a compressed structured data is not fun, and there is a bunch of
  %   compilers that do that (bunch of them for sparse and only one for arbitrary structured data). But how can we certify that those computations are correct?
  % \item The process of verification begins with a well-defined specification. Therefore, our initial focus should be on understanding how to specify structured data formats. Additionally, to ensure that our verification approach is applicable to real-world examples, it is essential to be able to express the format encoding used by major applications, such as modern sparse/structured data compilers \vg{TODO:\@ citations}. 
  % \item One common way to encode such formats is the use of special Domain-Specific Languages (DSLs). These DSLs are designed specifically for compiling efficient implementations of operations on structured data. In case of \finch cases, these DSLs may incorporate statefulness to express more formats in a more compact way.
  % \item To address the challenges posed by diverse data formats and stateful DSLs, we must establish the following objectives:
  % \begin{itemize}
  %   \item Develop a logic that is capable of expressing the correctness of operation implementations on structured data, where the structure of the data is defined by a stateful program.
  %   \item Create a set of rules that facilitate convenient and straightforward reasoning within this logic. 
  % \end{itemize}
  % \item However, if we want systematically incorporate such way of format description (we call them ``format'' functions further), it is naturally necessary to fix how imperative programs actually represent such data. This entails determining the input required by these format functions and the desired output they should produce.
  % \item One initial approach that comes to mind is to treat a format function as a program, which would take format components and generate a resampled version of the data in a ``dense'' form, in other words form where no compression is applied.
%  \end{itemize}
  
  


 
  % \item Show a very first small example: Run-Length format, and a naive approach of its verification using vanilla Separation logic. In this simple case we represent our format via predicate.
  % \item How did we came up with that predicate? Well, we had a verbal description of the format, so we just formalized that description in logic. 
  % \item Is there way of format decryption which
  % \item 
  %   \begin{itemize}
  %     \item is systematic
  %     \item is used by modern compilers, such that we would be able to verify their results
  %   \end{itemize}
  % \item Well, modern compilers often use DSL to describe such formats. In case of finch that DSL can contain arbitrary imperative code.
  % \item So we propose a logic a logic where one can describe formats using arbitrary imperative code. So it is possible to capture any DSL-like description 
  % \item But what this imperative description of formats should do? What should be its input and output?
  % \item Fist approach that leads to vanilla hyper-triples is  to treat our format description as a program that, given a sparse representation components, outputs you the dense tensor. In our case of a dense vector it. Show the RL example
  % \item 
%\end{itemize}




% \is{Some old ideas on the intro below}

% \paragraph{Motivation}

% Here comes the mighty example that illustrates the need for
%   first-class components in the triples, which is currently not the
%   case in existing hypersafery logics.

% The analogy is like to be able to write a program with fixed $k$
% procedures vs a program that is parameterised by $k$ and generates
% procedures with it. 

% Difference with Derek \etal's work:
% \begin{itemize}
% \item The allow for mixing hyper-triples of different fixed arity, so
%   do we.
% \item They do not arity-parametric specifications as well as the use
%   of symbolic component indices in the triples. This is crucial
%   crucial when provide a specification involving a non-constant number
%   of components. As an example, consider an effectful \code{mapi f l}
%   funciton, where each iteration of the effectful function sets an
%   element of some array to an index.

% \item We recognise the need for such specs in verifying manipulations
%   with multiple instances sparse data. \todo{Explain why we need a
%     program per data instance.}
% \end{itemize}






% \is{Some thoughts on the intro structure below}

% Main message of the introduction:

% \begin{itemize}
% \item Hoare logics for hypersafety~\cite{DOsualdoFD22} can be used for
%   simple optimisations, and are all around great.
% \item \textbf{Motivation:} Lowering in compilers is difficult to reason about, and existing
%   hyperlogicsare inadequate for our purposes (example!).
% \item \textbf{Key Ideas:} \emph{Parameterised} hypersafety is what we need: when the component
%   indices are truly first-class in the specifications.
% \item In addition, non-lockstep loops are tricky
% \item We build a logic for this and prove its sound
% \item We also show how to verify the results of a state-of-the-art
%   compiler \finch
% \end{itemize}



% \begin{figure}
%   \begin{subfigure}[b]{0.3\textwidth}
%     \centering
%     \small
%     \begin{minted}{python3}
%       def dot_prod(x_ind, x_val, y_ind, y_val, ans)
%         iX, iY, step = 1, 1, 0
%         while (iX < x_ind.length() && iY < y_ind.length()):
%           stride := min(x_ind[iX], y_ind[iY])
%           for i in range(step, stride):
%             ans[i] := x_val[iX] * y_val[iY]
%           iX += stride == x_ind[iX]
%           iY += stride == x_ind[iY]
%           step := stride
%     \end{minted}  
%     \caption{Dot product implementation}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[b]{0.3\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{img.png}
%     \caption{Dot product illustration}
%   \end{subfigure}

% \begin{center}
%   \small
%   \begin{minted}{python3}
%     def RL(x_ind, x_val)
%       x := new[N]
%       for i in range(0, x_ind.length()-1):
%         for j in range (x_ind[i], x_ind[i+1]):
%           x[j] := x_val[i]
%       return x
%   \end{minted}  
% \end{center}
% \end{figure}

% \begin{itemize}
% \item Structured data is eating the world, it's absolutely everywhere (ML,
%   routing, \etc).
% \item Computing on structured data is not fun, and there is a bunch of
%   compilers that do that (bunch of them for sparse and only one for arbitrary structured data). But how can we specify that those computations are correct?
% \item The key challenge in such reasoning comes from the definition of
%   the format, which makes such computations so complex.
% \item One way to specify a format is via a predicate. Let's take a look at a small example of an array with repeated values. Vector $X$ is said to be represented in a Run-Length Format via two arrays $x_{ind}$ and $x_{val}$ if for all indices $i$ in between $x_{ind}[j]$ and $x_{ind}[j+1]$ for some $j$, $X(i) = x_{val}(j)$~\ref{img:rlf}.


% In other words $x_{ind}$ stores coordinates of all chunks with repeated data in $X$, and $x_{val}$ stores corresponding values. Now consider a function that takes a summation of all elements in $X$
% \begin{center}
%   \small
%   \begin{minted}{python3}
%     def sum(x_ind, x_val):
%       for i in range(0, length(x_ind))
%         s += x_val[x_ind[i]] * (x_ind[i+1] - x_ind[i])
%   \end{minted}
% \end{center}

%   We can specify the correctness of it in a simple separation logic 
%   \[ \hsll
%     {\arr{x_{ind}}{x_{ind}} \strnl \arr{x_{val}}{x_{val}} \strnl P(X, x_{ind}, x_{val})}
%     {\mathtt{sum(x_{ind}, x_{val})}}{s}{s = \sum_i X(i) \str \top} \]

%   % One way to specify a format is via a predicate (give a
%   % hypothetical example). This will allow to use standard unary
%   % Hoare-style frameworks, such as separation logic, but writing format
%   % specifications in such style is unnatural (although this is a nice
%   % future work, so let's remember this point).
% \item However, in general case, formats for representing structured arrays could be arbitrary complex. In order to have a uniform way of representing a large class of them it is often necessary to build a DSL specifically designed to represent such formats~\cite{ArnoldHKBS10,AhrensDKA23}. In the later work such formats might even contain arbitrary pieces of imperative code. But how can we even specify the correctness of the implementation of an operation in the case when our formats are presented as a stateful programs?

%   % \vg{TODO} (Here comes the motivation) Another, more friendly way is to
%   % specify formats in a some sort of domain specific language that
%   % tells how to restore \emph{dense} representation from a sparse one
%   % (citations!)
% \item One and the most naive way would to treat our format description as a program that, given a sparse representation components, outputs you the dense tensor. In our case of a dense vector it would look like 
% \begin{center}
%   \small 
%   \begin{minted}{python3} 
%   def RL(x_ind, x_val)
%     x := new[N](0)
%     i := 1
%     for k in (0, N):
%       if k >= x_ind[i]:
%         i++
%       x[k] = x_val[i]
%     return x
% \end{minted}
% \end{center}
%   % For instance, this is how one can specify a sparse vector
%   % (example), and this is how computing a sum of elements over it looks
%   % like (example).
% \item \vg{TODO} Now, we can phrase the verification problem for our summation
%   program as the following \emph{hyper-safety} specification
%   \[\hsll{
%         \arr{x_{ind}(1)}{x_{ind}} \strnl \arr{x_{val}(1)}{x_{val}} \strnl
%         \arr{x_{ind}(2)}{x_{ind}} \strnl \arr{x_{val}(2)}{x_{val} }}
%         {1: & \mathtt{sum(x_{ind}, x_{val})} \\
%          2: & \mathtt{RL(x_{ind}, x_{val})}}{s \\ x}
%         { \exists a, \\ \ \arrl{x(1)}{a} \strnl s = \sum_i a(i) \strnl \top }\]
% \item \vg{TODO} A paragraph on what is the state of the art in program logics
%   for hypersafety (PLHS). \\ The proof in the PLHS framework can indeed be done, but it needs a sophisticated form of reasoning known as loop alignment. The complexity of this reasoning arises due to the following fact: within the $\mathtt{sum}$ loop, each iteration performs a summation of a substantial portion of repeated values within the vector $X$. Consequently, to establish the proof, each iteration of the $\mathtt{sum}$ loop must be aligned with a specific number of iterations within the $\mathtt{RL}$ loop.

%   As the complexity increases, particularly when dealing with more advanced formats of structured data, the alignments between these loops become more and more convoluted \vg{we provide example vere it gets very convoluted in subsecuent sections}. Hence, taking into account the inherent complexities associated with loop alignment \vg{cite all this differential privacy papers with crazy loop alignment rules}, it is clear that such proofs, conducted in PLHS, might become tedious and intricate.

%   We present a novel enhancement to the conventional PLHS framework that effectively addresses the aforementioned challenge. Our proposed approach revolves around a fundamental idea: rather than computing each element of the structured array sequentially within a loop and subsequently facing the challenge of aligning this loop with the corresponding loop in the ``client'' program, we propose an alternative strategy. Our approach involves computing each element of the structured array independently and then grouping batches of such computations with a specific number of iterations from the ``client'' loop.

%   The intuition behind this approach stems from the inherent nature of loop iterations, which are typically designed to be executed in a specific order. By regrouping such computations, the requirement of maintaining additional invariants associated with the order of execution arises. Consequently, rearranging portions of independent executions becomes a relatively simpler task, as the specific order in which these computations are performed does not matter anymore.

%   Now we show how to apply this idea in practice via \emph{parametrizing} hyper-triples

%   First we rewrite the representation of the $\mathtt{RL}$ format as follows:
%   \begin{center}
%     \small
%     \begin{minted}{python3}
%     def RL(x_ind, x_val, i)
%       k = 0
%       while x_ind[k] < i:
%           k++
%       ret x_val[k]
%     \end{minted}
%   \end{center}
%   This code, given an index $i$, computes the correspondent element of vector $X$.
%   % \vg{TODO} (Key ideas start here) The limitation of existing PLHSs is that
%   % they don't treat indices as first-class citizens. Why this is even
%   % needed for our problem?
% \item But how are we going to proceed with a specification? The problem is that now the specification should involve $\mathtt{RL(x_{ind}, x_{val},i)}$ for all $\mathtt{i}$ in the correspondent dimensional bounds.

% So our post condition should contain something like that:
% $$ s = \sum_i x(i) $$

% Where $x(i)$ is the output of $\mathtt{RL(x_{ind}, x_{val}i)}$ and $s$ is an output of $\mathtt{sum(x_{ind}, x_{val})}$. To cape this issue we introduce \emph{parametrized} hyper-triple, in which, instead of running a fixed amount of programs, we can run a whole family of them, parametrized by indices form some finite set. That is our first key contribution.\@ So we can rewrite our specification as follows:
% \[\hsll
%   {\arr{x_{ind}(*)}{x_{ind}} \strnl 
%    \arr{x_{val}(*)}{x_{val}}}
%   {1:              & \mathtt{sum(x_{ind}, x_{val})} \\
%    2: i \in [0, N] & RL(x_{ind}, x_{val},i)}
%   {s \\ x}
%   {s = \sum_i x(i) \str \top}\]
% % \[\hsll{}
% %         {1: & \mathbb{C} \\
% %          2: & \mathtt{CSR()}}{\_ \\ x}
% %         { \arr{y(1)}{X \cdot V} \strnl \arrtwo{x}{X} \strnl \top }\]
%   % \vg{TODO} Well, the key is in \emph{mixing} declarative and imperatie
%   % components of the format descriptions, so we could rewrite our
%   % specification as a \emph{parametrized} hyper-triple. Giving logical
%   % support for such parametrised triples is our first key idea.
% \item Now, nevertheless, $\mathtt{RL}$ still contains a loop, we will organize our logic in such a way, that this loop will not have to be aligned with other loops. It comes form the fact, each iteration on the $\mathtt{sum}$ loop, corresponds to bunch of independent executions of $\mathtt{RL}$. Hence, reasoning about $\mathtt{RL}$ loop, will be very much similar to as it was done in a simple separation logic. Providing such a proof system, is our second key contribution.
%   % (why? intuition
%   % needed), but we still have a loop in the ``client'' program. Our
%   % second key idea has to do with how to deal with the loop.
% \item \vg{TODO} Further, while ``formats'' can be all expressedn in terms of folds,
%   ``clients'' might have \code{while-loops}, hence we need more rules.
% \item (Contributions paragraph) With all that, we our contributions
%   are as follows. 
%   \begin{itemize}
%   \item Formulation of specification verification of computations with
%     sparse data as hyper-properties over a parametric number
%     (non-constant) of components.
%   \item An generalisation of the logic by d'Osualdo a (1) separation
%     logic that (2) supports parametric arity and (3) features a new
%     set of rules for restructuring loops
%   \item Mechanisation of the logic in Coq based on CFML memory model
%   \item Demonstration of the logic's utility on a series of
%     challenging benchmarks that were never previously formally
%     verified (using a program logic or otherwise)
%   \end{itemize}
% \item Paper outline (space permitting)
% \end{itemize}


==> leftovers.tex <==
\section{Introduction}

As a motivating example we consider a program that computes a product of a dense matrix and and a dense array compressed with some two arbitrary structured data formats (denote them as \code{mf} and \code{vf}). 
%
The first question we have to answer is how to specify this function. To figure out what would be the best and the cheapest way to do it, we have analyzed some major state-of-the-art libraries containing modules for sparse tensor computations like \tname{SciPy} (Python), \tname{CsMatBase} (Rust), \tname{Eigen} (C++) \etc. \vg{Links?} We noticed that all of those libraries among other things offer implementations of random access methods for targeted compressed structures. Other than that, the recent work by \citeauthor{AhrensDKA23}, present a stateful language \looplets to describe structured data formats. Programs in this language can be seen, as a random access format's methods as well.
%
Being generally useful, random access functions demonstrate the way how one should think about the format: they describe a way how to restore one particular element of the data in the traversal that follows the structure of its compression. Having this in mind we claim, that random access functions are good fit for clear specifications and proofs as well.


%
Let's see how can we specify our motivating example in such terms. First, we consider two random access functions for our two formats: \code{m_get} for the matrix and \code{v_get} for the vector. Their signatures are presented on~\autoref{fig:sigs}. \code{m_get} takes a structure that represent compressed matrix \code{m:mf} and \code{v_get} takes a compressed vector \code{v:vf}. Typically, those structures store a tuple of arrays with their sizes. Then, \code{m_get} takes two indexes (row and column position) and returns a value by those positions (of some type \code{val}). In the same time \code{v_get} takes only one index (position in the vector) and returns a value of the same type.
%
The signature of the function we are going to verify, product function \code{mv_prod} follows the same logic. It takes compressed matrix and vector and outputs the array filled with their product values (\code{val[]}). We will get back to its general implementation scheme later. 


Now let's understand how we can specify \code{mv_prod} in terms of
\code{m_get} and \code{v_get}. To do that, note that morally
specification for \code{mv_prod}, should relate its outcome with
elements of dense representations of \code{m} and \code{v}. Those
elements can be retrieved by calling \code{m_get} and \code{v_get} on
the set of all indexes bounded by sizes of given matrix and vector. It
suggests us to construct our specification by relating the output of
\code{mv_prod} with all outputs of \code{m_get} and \code{v_get}. 
%

So-called \emph{relational} program logics are a well-studied formalism to specify and reason symbolically about hypersafety properties of programs~\cite{Benton04,BartheCK11,Yang07}.
%
The applications of such logics range from proving algebraic properties of stateful programs~\cite{SousaD16} and specifying validity of program optimisations~\cite{CarbinKMR12} to reasoning about information flow security~\cite{NanevskiBG11} and differential privacy~\cite{BartheKOB12}.


Precondition features the predicate $P_{\code{mf}}$ (\emph{resp}.~$P_{\code{vf}}$). When applied to a pointer \code{p}, this predicate ensures that \code{p} points to a structure which encodes the compressed matrix (\emph{resp}.~vector) \wrt to \code{mf} (\emph{resp}.~\code{vf}) format. The syntax $(\cdot)$ in $\Pm$ (\emph{resp}.~$\Pv$) in the precondition is used to indicate distinct copies of the same predicate across multiple state components indexed by elements of $\set{1}\cup \set{\angled{2,i,j} : i \in [0,N)\, j \in [0,M)}\cup\set{\angled{3,j} : j \in [0,N)}$. The latter set in called the index set of the triple. An independent run with each index~$i$ runs on the copy of the heap with the same index. Finally, the post-condition ensures that the output of the first component $a$, is a pointer, pointing to an array with content $s$, which is pointwise equal to the dot product of given matrix and vector.






Before we dive into the general proof flow of~\eqref{eq:mv_prod} making use of the parametrised nature of of specification, lets discuss the general implementation scheme of \code{mv_prod} (\autoref{fig:sigs} (lines~8-9)). Typically, each complex tensor compression format relies on the a simpler compression of its parts. For example a lot of matrix compression formats like Compressed Sparse Row (CSR), Doubly Compressed Sparse Row (DCSR), Linked List (LIL) \etc first independently compress each row of the matrix, and then assemble those compressions into one structure. As such, a typical implementation of \code{mv_prod} would start with partitioning the matrix \code{m} into its components \code{mp}, encoded with a simpler formats (line~8), and multiplying each of them by a vector \code{v} (line~9).

Note that each part \code{mp} covers elements only some subset of elements of the original matrix \code{m}. Such subset might be the set of elements from a particular row. Intuitively this induces a partition on the set of indexes of \code{m}'s elements. More formally, the set of indexes of elements from \code{m} can be partitioned as follows: 
{\small{\( \angled{2,i,j}_{i \in [0,M),\, j \in [0,N)}  = S_\emptyset \cup \bigcup_{i = 1}^{K} S_i  \)}}, where $S_\emptyset$ correspondence to the set of indexes which don't belong to any element of the partition (for example, set with zero elements of the matrix), and each $S_i$ corresponds to the set of indexes covered by \code{mp} on the $i$\ith iteration. Then \logic allows us to reduce the verification of~\eqref{eq:mv_prod} to verification of the following hyper-triples:

\begin{equation}
  \label{eq:mv_prod1}
  {\small{
    \hspec{\!
  \begin{array}{l}
    \Pm \str\\[2pt]
    \Pv
  \end{array}
  \!\!}    
  \hmid{\!\!\!
    \begin{array}{c@{\ }c@{\ }l}
    \angled{2, i, j}_{\!\!\!\!\tiny
      \begin{array}{l} i \in S_\emptyset \\ j \in [0,N) \end{array}} \!\!\!\!\!:  \mathtt{m\_get(m,\ } i,\ j)
    \end{array}
  \!}
  \hspec{\!\!\!
  \left.
  \begin{array}{r}
  \many{m}
  \end{array}
  \right|
  \begin{array}{l}
  \many{m}=\many{0}
  \end{array}
  \!\!\!}
  }}
\end{equation}

which is a hyper-triple that handles zero values removed with the compression, and a hyper-triple that handles values from each~$S_k$, where~$k$ goes from~$1$ up to~$K$:

\begin{equation}
  {\small{
   \hspec{\!
  \begin{array}{l}
    \Pm \str\\[2pt]
    \Pv
  \end{array}
  \!\!}    
  \hmid{\!\!\!
    \begin{array}{c@{\ }c@{\ }l}
    1 &:& \mathtt{inner\_prod(mp, v)} 
    \\ [2pt]
    \angled{2, i, j}_{\!\!\!\!\tiny
      \begin{array}{l} i \in S_k \\ j \in [0,N) \end{array}} &:&  \mathtt{m\_get(mp,\ } i,\ j)
    \\ [2pt]
    \angled{3, j}_{j \in [0, N)} &:& \mathtt{v\_get(v,\ } j)
    \end{array}
  \!}
  \hspec{\!\!\!
  \left.
  \begin{array}{r}
  a \\[2pt] \many{m} \\[2pt] \many{v}
  \end{array}
  \right|
  \begin{array}{l}
  \arrl{a}{\many{m}\cdot\many{v}}
  \end{array}
  \!\!\!}}}
\end{equation}
%
Parametrised hyper-triples give us a flexibility to align independent random access functions with the operation code in any way we like. This benefit is especially visible when the format \code{mf} assumes some non-trivial partition into subparts. For example unordered Compressed Sparse Row (uCSR) format, stores the encoding of each row in some arbitrary order which is determined by a special array \code{idx}. Hence, the efficient implementation of \code{mv_prod} would iterate over those row in the order determined by \code{idx}. To align \code{m_get} functions in this case, one will have to partition the index set as \(\bigcup_{i =0}^{|\code{idx}|} S_{\code{idx}[i]} \), where $S_i$ is a set of indexes for each row.
%
Moreover, as all runs of \code{m_get} are independent, the price of all such alignments is cheap: we will only have to prove the sets equality, the implementation of the \code{m_get} itself, as well ass the heap state are irrelevant here.
\vg{Move to discussion?}
\begin{wrapfigure}[6]{r}{0.30\textwidth}
  \vspace{-15pt}
  \begin{minted}[numbers=left, xleftmargin=2.5ex, numbersep=6pt, escapeinside=@@, fontsize=\footnotesize]{python3}
  for i in range(0,N):
    for j in range(0,M):
      x[i,j] = m_get(i,j)
  \end{minted}
  \setlength{\abovecaptionskip}{10pt}  
  \caption{Rolling all \code{m_get} runs into one loop}
  \label{fig:lhc}
\end{wrapfigure} 
In contrast, trying to mimic the same types of alignment in such logics as LHC without the parametrisation will exacerbate the complexity of proofs. One appealing way to model \logic proofs in LHC would be to ``roll'' all independent runs of random access functions into one loop, that populates a dense array with the results of \code{m_code}, and uses this array in the post-condition instead of $\many{m}$. The disadvantage of such approach is that, whenever one wants to reorder the executions of \code{m_get}, they will have to justify that such reordering will be indeed sound. Such proofs will depend on the heap-state and \code{m_get} itself.


\begin{wrapfigure}[6]{r}{0.42\textwidth}
\setlength{\abovecaptionskip}{7pt}
\vspace{-10pt}
\begin{minipage}{1\linewidth}
{\small{
  \begin{prooftree}
    \AXC{idx\((Q_1) \subseteq \text{supp}(t_1)\ \) idx\((Q_2) \subseteq \text{supp}(t_2)\)}
    \noLine
    \UIC{\(\mathsf{wp}\ t_1 \{ Q_1 \} \land \mathsf{wp}\ t_2 \{ Q_2 \}\)}
    \RightLabel{\small \tname{Wp-Conj}}
    \UIC{\( \mathsf{wp}\ (t_1+t_2)\ \{Q_1 \land Q_2 \} \)}
  \end{prooftree}
}}
\end{minipage}
\caption{\tname{Wp-Conj} rule from LHC} 
\label{wpconj} 
\end{wrapfigure}
Finally, \logic is a separation logic (SL), while LHC is a Hoare logic
defined over a finite set of distinct variables.
%
We conjecture that generalising LHC to SL would present some
challenges.
%
For example, consider one of the key LHC rules \tname{Wp-Conj}
(\autoref{wpconj}).
%
This rule allows one to conjoin specifications of two program products
$t_1$ and $t_2$ with possibly overlapping components, yielding
$t_1 + t_2$, if $t_1$ and $t_2$ agree on the overlapping part.
%
Generalising this rule for SL-style assertions would require to
introduce extra restrictions for using the plain
conjunction~\cite{GOTSMAN2011171}.
%
In~\autoref{sec:merge}, we have shown a solution to that problem
implemented in \logic.
%
Given specifications of program products with overlapping (but
differently indexed) parts $\hslcc{H_1}{S_1:\pp_1}{Q_1}$ and
$\hslcc{H_2}{S_2:\pp_2}{Q_2}$, one can first combine them using the
\tname{Seq} rule from~\autoref{fig:struct-rules}, yielding a triple
with duplicated components
$\hslcc{H_1\!\str\!H_2}{S_1:\pp_1,\ S_2:\pp_2}{Q_1\!\str\!Q_2}$, and
then use the \tname{Merge} rule to get rid of the duplicates.



% \input{figtriples}
\begin{figure}[t]
  %\setlength{\belowcaptionskip}{-15pt}
    % \begin{tabular}{c}
    %   \begin{minipage}{0.48\textwidth}
    %     \vspace{2mm}
    %     {\small{
    %       \includegraphics[width=0.8\linewidth]{figures/altogether2.pdf}
    % }}
    % \end{minipage}
    % \\\\[-5pt]
    % \begin{minipage}{0.48\textwidth}
      % \vspace{-30mm}
        % {\small{\mathfrak{B} 
          \begin{lstlisting}[language=Coq,xleftmargin=0pt,xrightmargin=0pt,basicstyle=\scriptsize\ttfamily,numbersep=5pt]
Lemma spec_spmspv (midx mind mval xind xval : loc) :
{{ Arrs }} [{
  [1| _  \in {0}           => spmspv midx mind mval xind xval];
  [2| ij \in [0,M) \x [0,N) => uscr_get midx mind mval ij.1 ij.2];
  [3| j  \in [0,N)         => sv_get xind xval j];
}] {{ a m x, arr(a, fun i => \sum_(j \in [0, N)) m(i,j) * x(j) }}
Proof. xstart. (* proof start *)
  (* \ss 2.1.1 *)
  xin (1,0) : xmalloc p=> //; xret.
  (* \ss 2.2 *)
  xfocus 2 (indom (midx \x [0, N) )).
  (* \ss 2.1.2 *)
  xapp spec_ucsr_get.
  - case=> ??; indomE; tauto.
  xclean_unused. (* clean up unused assertions *)
  (* frame out unused part of ans array *)
  xframe_array p midx.
  - move=> *; erewrite <-Sum0s at 1; apply/SumEq=> ?.
    by indomE=> /=; case_if.
  (* partition index set into Si to apply For-rule *)
  have E: [0,M)\x[0,N) \cap midx\x[0,N) = midx\x[0,N)
  - rewrite prod_intr_list; f_equal; exact/intr_list.
  rewrite E fset_of_list_nodup prod_Union_distr.
  rewrite -(Union_same |midx| [0, N)).
  (* \ss 2.3 *)
  xfor with Inv := inv.
  - xin 2: xapp spec_index; xstep; xif=> [?|]; xgo. 
    xin 1: xgo.
    rewrite index_nodup //; try math. (* simplify goal *)
    (* \ss 2.4 *)
    xsubst (fun (2,i,j) => (2,j)).
    (* \ss 2.5 *)
    xapp spec_spvspv.
    xsimpl=>->; xstep; xsimpl*. (* store result of spvspv *)
\end{lstlisting}
\vspace{-3mm}
\begin{lstlisting}[numbers=none,language=Coq,xleftmargin=0pt,xrightmargin=0pt,basicstyle=\scriptsize\ttfamily,numbersep=5pt]
  (* solve arithmetic to adjust big summations in precondition *)
\end{lstlisting}
\vspace{-3mm}
\begin{lstlisting}[firstnumber=42,language=Coq,xleftmargin=0pt,xrightmargin=0pt,basicstyle=\scriptsize\ttfamily,numbersep=5pt]
Qed.
\end{lstlisting}
      % }}
      % \end{minipage}
  % \end{tabular}
  \caption{Derived rules for sequential composition and independent products.}  
  \label{fig:seq}
  \end{figure}


\input{figtriples}

==> semantics.tex <==

\section{Soundness of the Logic}
\label{sec:semantics}


